Cross-model Back-translated Distillation for Unsupervised Machine Translation

Recent unsupervised machine translation (UMT) systems usually employ three main principles: initialization, language modeling and iterative back-translation, though they may apply them differently. Crucially, iterative back-translation and denoising auto-encoding for language modeling provide data diversity to train the UMT systems. However, the gains from these diversification processes has seemed to plateau. We introduce a novel component to the standard UMT framework called Cross-model Back-translated Distillation (CBD), that is aimed to induce another level of data diversification that existing principles lack. CBD is applicable to all previous UMT approaches. In our experiments, CBD achieves the state of the art in the WMT'14 English-French, WMT'16 English-German and English-Romanian bilingual unsupervised translation tasks, with 38.2, 30.1, and 36.3 BLEU respectively. It also yields 1.5-3.3 BLEU improvements in IWSLT English-French and English-German tasks. Through extensive experimental analyses, we show that CBD is effective because it embraces data diversity while other similar variants do not.

==> img/Sbackground.tex <==
\section{Background}\label{sec:background}


\citet{ravi2011deciphering} were among the first to propose a UMT system by framing the problem as a \textit{decipherment} task that considers non-English text as a cipher for English. Nonetheless, the method is limited and may not be applicable to the current well-established NMT systems \citep{luong2015effective,vaswani2017attention,payless_wu2018}. \cite{lample2017unsupervised} set the foundation for modern UMT. They propose to maintain two encoder-decoder networks simultaneously for both source and target languages, and train them via denoising auto-encoding, iterative back-translation and adversarial training. 
% After that, \citet{lample2018phrase_unsup} formulated a framework for UMT with three principles that can be customized: 
{In their follow-up work,  \citet{lample2018phrase_unsup} formulate a common UMT framework for both PBSMT and NMT with three basic principles that can be customized.} The three principles are: % from Lample paper: "Given the ill-posed nature of the task, model initialization expresses a natural prior over the space of solutions we expect to reach, jump-starting the process by leveraging approximate translations of words, short phrases or even sub-word units (Sennrich et al., 2015b).
\begin{itemize}[leftmargin=*,itemsep=0.5pt]
    \item \textbf{Initialization}: A non-randomized {cross- or multi-lingual} initialization that represents a knowledge prior to bootstrap the UMT model. For instance, \citet{lample2017unsupervised} and \citet{effective-artetxe-etal-2019} use an {unsupervised} word-translation model MUSE \citep{muse_conneau2017word} as initialization to promote word-to-word {cross-lingual} transfer. {\cite{lample2018phrase_unsup} use a shared jointly trained sub-word \citep{sennrich2015neural} dictionary.} On the other hand, \citet{conneau2019cross_xlm} use a pretrained cross-lingual masked language model (XLM) to initialize the unsupervised NMT model. %\blue{You might need to clarify it more..}
    
    \item \textbf{Language modeling}: Training a language model on monolingual data helps the UMT model to generate fluent texts. The neural UMT approaches \citep{lample2017unsupervised,lample2018phrase_unsup,conneau2019cross_xlm} use denoising auto-encoder training to achieve language modeling effects in the neural model. Meanwhile, the PBSMT variant proposed by \citet{lample2018phrase_unsup} uses the KenLM smoothed n-gram language models \citep{pbsmt_lm_heafield2011kenlm}.

    \item \textbf{Iterative back-translation}: Back-translation \citep{backtranslate_sennrich-etal-2016-improving} brings about the bridge between source and target languages by using a backward model that translates data from target to source. The {(source and target)} monolingual data is translated back and forth {iteratively} to {progress} the UMT model in both directions.
\end{itemize}


During training, the initialization step is conducted once, while the denoising and back-translation steps are often executed in an alternating manner.\footnote{{The KenLM language model in PBSMT \citep{lample2018phrase_unsup} was kept fixed during the training process.}} It is worth noting that depending on different implementations, the parameters for backward and forward components may be separate \citep{lample2017unsupervised} or shared \citep{lample2018phrase_unsup,conneau2019cross_xlm}. A {parameter-shared} cross-lingual NMT model has the capability to translate from either source or target, while a UMT system with parameter-separate models has to maintain two models. 
Either way, we deem a standard UMT system to be bidirectional, i.e. it is capable of translating from either source or target language.
% ERROR: \ie\ cause error, just do manually i.e.


% In either way, we deem an encapsulated UMT system built by the three principles as \red{bidirectional} in this paper.

Our proposed cross-model back-translated distillation (CBD) works outside this well-established framework. It employs two UMT agents to create extra diversified data apart from what existing methods already offer, rendering it a useful add-on to the general UMT framework. Furthermore, different implementations of UMT as discussed above can be plugged into the CBD system to achieve a performance boost, even for future methods that may potentially not employ the three principles.
% related works at the bottom


\begin{comment}

\citep{pbsmt_Koehn:2003:SPT}
\citep{scaling_nmt_ott2018scaling}

\citep{vaswani2017attention}
\citep{payless_wu2018}
\citep{sennrich2015neural}
\citep{luong2015effective}
\citep{muse_conneau2017word}
\citep{nguyen2019data}
\citep{knowledge_distill_kim_rush_2016}
\citep{kim2016sequence_knowledge_distillation}
\citep{denoising_ae_vincent2008extracting}
\citep{ensemble_distill_freitag2017}
\citep{effectove-artetxe-etal-2019}
\citep{devlin2018bert}
\citep{lample2017unsupervised}
\citep{lample2018phrase_unsup}
\citep{conneau2019cross_xlm}

\citep{fasttext,word2vec_mikolov2013distributed}
\end{comment}











==> img/Sexperiments.tex <==

We present our UMT experiments on the WMT tasks (\cref{subsec:wmt}) followed by IWSLT (\cref{subsec:iwslt}). 

\subsection{WMT experiments}\label{subsec:wmt}



\paragraph{Setup.} We use the default data setup and codebase of \citet{conneau2019cross_xlm}'s code repository\footnote{\href{https://github.com/facebookresearch/XLM}{https://github.com/facebookresearch/XLM}}. Specifically, we use the News Crawl 2007-2008 datasets for {English (En)}, French (Fr) and German (De), and News Crawl 2015 dataset for Romanian (Ro), and limit the total number of sentences per language to 5M. This results in a total 10M, 10M and 7M sentences of {combined} monolingual data for En-Fr, En-De and En-Ro, respectively. Note that in their paper, \cite{lample2018phrase_unsup} and \cite{conneau2019cross_xlm} conducted their UMT experiments on very large datasets of 274M, 509M and 195M sentences {(combination of source and target monolingual data)} for En-Fr, En-De and En-Ro respectively, which are derived from News Crawl 2007-2017 datasets. Unfortunately, we were unable to reproduce these (very) large scale experiments because we encountered out-of-CPU-memory error when attempting to load the large datasets, even though our system has 128GB RAM. Instead, we rerun the NMT and PBSMT models \citep{lample2018phrase_unsup} and the pretrained XLM \citep{conneau2019cross_xlm} on the default setup to acquire the corresponding {NMT, PBSMT and XLM} baselines. 



%Note that in their paper, \citet{lample2018phrase_unsup,conneau2019cross_xlm} conducted their UMT experiments on astronomically large datasets of 274M, 509M and 195M sentences for En-Fr, En-De and En-Ro respectively, which are derived from News Crawl 2007-2017 datasets. Unfortunately, we were unable to reproduce these (very) large scale experiments \blue{because we encountered out-of-CPU-memory error when attempting to load the large datasets, even though our system has 128GB RAM}. Instead, we use the News Crawl 2007-2008 datasets for English and German, and 2015 dataset for Romanian, and limit the total number of sentences per language to 5M, which is actually the default setup in \citet{conneau2019cross_xlm}'s code\footnote{\href{https://github.com/facebookresearch/XLM}{https://github.com/facebookresearch/XLM}}. This results in 10M, 10M and 7M sentences of {bilingual} monolingual data for En-Fr, En-De and En-Ro, respectively. We rerun the NMT and PBSMT models \citep{lample2018phrase_unsup} and the pretrained XLM \citep{conneau2019cross_xlm} on these reduced datasets to acquire the baselines.


For the NMT models, we follow \citet{lample2018phrase_unsup} to train the UMT agents with a parameter-shared Transformer \citep{vaswani2017attention} that has 6 layers and 512 model dimensions and a batch size of 32 sentences. We use {joint} Byte-Pair Encoding (BPE) \citep{sennrich2015neural} and train fastText \citep{fasttext} on the BPE tokens to initialize the token embeddings. For the PBSMT \citep{pbsmt_Koehn:2003:SPT} models, {following \cite{lample2018phrase_unsup},} we use MUSE \citep{muse_conneau2017word} to generate the initial phrase table and run 4 iterations of back-translation. We subsample 500K sentences from the 5M monolingual sentences at each iteration to train the PBSMT models.\footnote{For PBSMT, \citet{lample2018phrase_unsup} subsampled 5M out of 193M sentences of monolingual data. For NMT, they train for 45 epochs, which is almost 60x longer than us with data size taken into account.\label{foot1}} To ensure randomness in the PBSMT agents, we use different seeds for MUSE training and {randomly} subsample different sets of data during PBSMT training. {For XLM \citep{conneau2019cross_xlm}, we also follow their setup. For each agent, we first pretrain a big XLM model (6 layers, 1024 model dimensions) on the default 10M data with 4K tokens per batch.}
Then we initialize the encoder-decoder system {of the UMT agent} with the XLM and train the model for 30 epochs.\footref{foot1} The NMT and XLM agents are trained with a 4-GPU setup. We use the big Transformer \citep{scaling_nmt_ott2018scaling} as the final supervised model. {We choose the best model based on validation loss and use beam size of 5.}



% Text with first footnote\footnote{\label{note1}This is the labeled footnote}
% and more text with a second footnote\footnote{here}.
% In this new paragraph we have a reference to the first
% footnote\footnotemark[\ref{note1}].

\begin{table}[h!]
\begin{center}
\vspace{-0.5em}
%\resizebox{0.9\textwidth}{!}{%
\caption{BLEU scores on WMT'14 English-French (En-Fr), WMT'16 English-German (En-De) and WMT'16 English-Romanian (En-Ro) unsupervised translation tasks.}
% \centering
\begin{tabular}{lcccccc}
\toprule
{\bf Method / Data}      & {\bf En-Fr} & {\bf Fr-En} & {\bf En-De} & {\bf De-En} & {\bf En-Ro}  & {\bf Ro-En}\\
\midrule
\midrule
\multicolumn{7}{l}{\bf Results reported from previous papers on large scale datasets}\\
\midrule
\textbf{Data Used}               & 274M  & 274M  & 509M & 509M & 195M  & 195M\\
\midrule
NMT \citep{lample2018phrase_unsup}                  & 25.1  & 24.2  & 17.2  & 21.0  & 21.1 & 19.4\\
PBSMT \citep{lample2018phrase_unsup}                & 27.8  & 27.2  & 17.7  & 22.6  & 21.3 & 23.0\\
% PBSMT + NMT \citep{lample2018phrase_unsup}          & 27.6  & 27.6  & 20.2  & 25.2  & 25.1 & 23.9\\
XLM \citep{conneau2019cross_xlm}         & 33.4  & 33.3  & 26.4  & 34.3  & 33.3 & 31.8\\
\midrule
\midrule
\multicolumn{7}{l}{\bf Results from our runs on smaller datasets}\\
\midrule
\textbf{Data Used}               & 10M  & 10M  & 10M & 10M & 7M  & 7M\\
\midrule
NMT \citep{lample2018phrase_unsup}                  & 24.7	& 24.5  & 14.5	& 18.2	& 16.7	& 16.3   \\
\hspace{1em} + CBD                                   & 26.5	& 25.8  & 16.6	& 20.4  & 18.3  & 17.7\\
\midrule
PBSMT \citep{lample2018phrase_unsup}                & 17.1	& 16.4	& 10.9	& 13.6	& 10.5	& 11.7	\\
\hspace{1em} + CBD                          & 21.6	& 20.6	& 15.0	& 17.7  & 11.3	& 14.5  \\
\midrule
XLM \citep{conneau2019cross_xlm}         & 33.0	& 31.5  & 23.9  & 29.3  & 30.6  & 27.9 \\
\hspace{1em} + CBD                          & {35.3}	& {33.0}  & {26.1}  & {31.5}  & 32.2   & 29.1 \\
% \midrule
% \multicolumn{7}{l}{\bf Multi-agent cross-translated diversification with multiplier $n=2$ on}\\
% NMT \citep{lample2018phrase_unsup}                  & 26.5	& 25.8  & 16.6	& 20.4  &  & \\
% PBSMT \citep{lample2018phrase_unsup}                & 	&   &   &   &  & \\
% Pretrained XLM \citep{conneau2019cross_xlm}         & 35.3	& 33.0  &   &   &  & \\
\bottomrule
\end{tabular}
% }
\vspace{-1em}
\label{table:main_results}
\end{center}
\end{table}


\paragraph{Results.} Table \ref{table:main_results} shows the experimental results of different UMT approaches with and without CBD. First of all, with the datasets {that are} 30-50 times smaller than the ones used in previous papers, the baselines perform around 2 to 3 BLEU worse than the reported BLEU. As it can be seen, the CBD-enhanced model with the pretrained XLM achieves 35.3 and 33.0 BLEU on the WMT'14 En-Fr and Fr-En tasks respectively, which are 2.3 and 1.5 BLEU improvements over the baseline. {It also surpasses \citet{conneau2019cross_xlm} by 1.9 BLEU}, despite the fact that the SOTA was trained with 274M sentences {(compared to our setup of {10M} sentences)}. CBD also boosts the scores for XLM in En-De, De-En, En-Ro, Ro-En by around 2.0 BLEU. For the NMT systems, CBD also outperforms the baselines by 1 to 2 BLEU. More interestingly, PBSMT models are known to be deterministic, but CBD is still able to improve data diversity and provide performance boost by up to 4.0 BLEU points.

% We used the Adam optimizer (Kingma and Ba, 2014) with a learning rate of 10−4 , β1 = 0.5, and a batch size of 32.

%\subsection{Small scale IWSLT'14 English-German and IWSLT'13 English-French}\label{subsec:iwslt}

\subsection{IWSLT experiments}\label{subsec:iwslt}
%  \red{Can we do an experiment with $k=3$?}
We also demonstrate the effectiveness of CBD on relatively small datasets for IWSLT En-Fr and En-De translation tasks. The IWSLT'13 En-Fr dataset contains 200K sentences for each language. We use the IWSLT15.TED.tst2012 set for validation and the IWSLT15.TED.tst2013 set for testing. The IWSLT'14 En-De dataset contains 160K sentences for each language. We split it into 95\% for training and 5\% for validation, and we use IWSLT14.TED.\{dev2010, dev2012, tst2010,tst1011, tst2012\} for testing. 
% {We choose the best model based on validation loss.}
For these experiments, we use the neural UMT method \citep{lample2018phrase_unsup} with a Transformer of 5 layers and 512 model dimensions, and trained using only 1 GPU. 

From the results in \Cref{table:ablation_iwslt}, we can see that CBD improves the performance in all the four tasks by 2-3 BLEU compared to the NMT baseline of \cite{lample2018phrase_unsup}.

% Since the datasets are small, we could afford to try out CBD with larger multipliers ($n=2,3,4$) and levels $k=3$. Thus, these experiments are also used for ablations to see what may be the best configuration for CBD. 

%We split 95\% and 5\% of the En-De dataset for train and valid sets, and  
% act as a ablation study 


\begin{table}[h!]
\begin{center}
% \vspace{-1em}
% \resizebox{\columnwidth}{!}{%
\caption{BLEU scores on the unsupervised IWSLT'13 English-French (En-Fr) and IWSLT'14 English-German (En-De) tasks.}
\begin{tabular}{lcccc}
\toprule
{\bf Method / Data}          & {\bf En-Fr} & {\bf Fr-En} & {\bf En-De} & {\bf De-En} \\
\midrule
NMT \citep{lample2018phrase_unsup}    & 29.6	& 30.7  & 15.8  & 19.1    \\
% \midrule
\hspace{1em} + CBD                  & 31.8 & 31.9  & 18.5  & 21.6    \\
% \hspace{1em} + CBD ($k=2,n=3$)                  & \textbf{32.8} & \textbf{32.2}  & \textbf{19.1}	& \textbf{22.2}       \\
% \hspace{1em} + CBD ($k=2,n=4$)                  & 32.3 & 32.1	& 19.1	& 22.1 \\
% \midrule
% \hspace{1em} + CBD ($k=3,n=3$)                  & 32.6 & 31.8	& 18.9	& 21.9 \\
\bottomrule
\end{tabular}
% }
% \vspace{-1em}
\label{table:ablation_iwslt}
\end{center}
\end{table}

% \paragraph{Results.} In \Cref{table:ablation_iwslt}, compare CBD againts the neural UMT baseline \citep{lample2018phrase_unsup} in the IWSLT setup. As shown, CBD improves the performance in all four tasks by 2-3 BLEU compared to the baseline.

% \vspace{-0.5em}
% \red{
% \paragraph{Results.} In \Cref{table:ablation_iwslt}, we compare different variants of CBD against the neural UMT baseline \citep{lample2018phrase_unsup}. As shown, 2nd level CBD with $n=2$ improves the performance in all four tasks by 2-3 BLEU compared to the baseline. Furthermore, increasing the multiplier to $n=3$ adds another 1 BLEU to the results. However, the experiments show that increasing it to $n=4$ does not improve the translation quality further. Furthermore, applying the 3rd level CBD seems to reduce the performance slightly, perhaps because the long daisy chain translation process induces more noises and deteriorates the sample quality.\footnote{We observed there are less duplicates in the 3rd level than the 2nd level CBD. There is also no performance change if we filter those duplicates. Thus, the performance drop in 3rd level is not due to less diversity.} Thus, scaling up CBD's synthetic parallel data may not always be beneficial; there is a saturation point that can be found through hyper-parameter tuning.
% }

% \red{Can we do an experiment with $k=3$?}


% \subsection{\red{Low-resource English-Nepali and English-Sinhala tasks}}

\vspace{-0.5em}
\section{Understanding CBD}\label{subsec:why_it_works}

% In this section, we investigate why CBD is able to improve the underlying UMT methods. 

%First, we test the performance of some sensible alternatives to CBD and explain why such methods do not improve the UMT systems. \red{Second, we show that the synthetic data generated by CBD are more diverse by comparing the reconstruction BLEU scores and the amount of duplicates in the data.}


% After that, we explain with experimental data why CBD is effective in improving performance by embracing data diversity and compare it with other similar variants as well as with ensembles of models.


\subsection{Cross-model back-translation is key} \label{subsec:cross_translation}


As mentioned, crucial to our strategy's success is the cross-model back-translation, where the agent operating at the first level must be different from the one in the second level. To verify this, we compare CBD with similar variants that do not employ the cross-model element in the WMT tasks. We refer to these variants {commonly} as \emph{back-translation distillation} (BD). The first variant \emph{BD (1st level,1 agent)} has only 1 UMT agent that translates the monolingual data only once and uses these synthetic parallel pairs to distill the model $\hat{\theta}$. The second variant \emph{BD (1st level, 2 agents)} employs 2 UMT agents, similar to CBD, to produce 2 sets of synthetic parallel data from the monolingual data and uses both of them for distillation. Finally, the third variant \emph{BD (2nd level, 2 agents)} uses 2 UMT agents to sample translations from the monolingual data in forward and backward directions using the same respective agents. In other words, BD (2nd level, 2 agents) follows similar procedures in \Cref{alg:macd}, except that it optimizes the following loss with $\theta_{\alpha}$ being alternated between $\theta_1$ and $\theta_2$:
% But instead of optimizing Eq. \ref{eqn:cbd_loss}, it optimizes the following loss:
% \begin{equation}
% \begin{aligned}
% \overline{\mathcal{L}}(\theta_{\alpha}, \hat{\theta}) &= -\E_{z\sim P(\cdot|y,\theta_{\alpha},t,s),y\sim P(\cdot|x,\theta_{\alpha},s,t),x\sim X_s} (\log P(y|x,\hat{\theta}) + \log P(y|z,\hat{\theta}))\\
%     &\quad -\E_{z\sim P(\cdot|y,\theta_{\alpha},t,s),y\sim P(\cdot|x,\theta_{\alpha},t,s),x\sim X_t} (\log P(x|y,\hat{\theta}) + \log P(z|y,\hat{\theta}))
% \end{aligned}
% \label{eqn:bd_loss}
% \end{equation}
\begin{equation}
\begin{aligned}
\overline{\mathcal{L}}(\theta_{\alpha}, \hat{\theta}) &= -\E_{z_s\sim P(\cdot|y_t,\theta_{\alpha}),y_t\sim P(\cdot|x_s,\theta_{\alpha}),x_s\sim \sX_s} \big[ \log P(y_t|x_s,\hat{\theta}) + \log P(y_t|z_s,\hat{\theta}) \big]\\
    &\quad -\E_{z_t\sim P(\cdot|y_s,\theta_{\alpha}),y_s\sim P(\cdot|x_t,\theta_{\alpha}),x_t\sim \sX_t} \big[ \log P(x_t|y_s,\hat{\theta}) + \log P(z_t|y_s,\hat{\theta}) \big]
\end{aligned}
\label{eqn:bd_loss}
\end{equation}

% \ie\
% As mentioned, crucial to CBD's success is cross-translation, where the agents operating at the current level must be different from those in the previous levels. To verify this, we compare CBD with other variants that do not employ cross-translation in the WMT tasks, which we refer to as \emph{multi-agent diversification} (MAD). The first variant \emph{MAD (1{\text{st}} level, $n=1$)} has 1 UMT agent in the 1st level that translates the monolingual data only once. The second variant \emph{MAD (1{\text{st}} level, $n=2$)} employs 2 UMT agents to produce 2 sets of synthetic parallel data from the monolingual data. Finally, the third variant \emph{MAD (2{\text{nd}} level, $n=2$)} uses 2 UMT agents to translate the monolingual data at level 1, and then uses the \emph{same respective agents} to back-translate those generated data to create level 2 data, \textit{i.e.,} $\gD$ is added with $(M_i^{t\rightarrow s}(M_i^{s\rightarrow t}(S)), M_i^{s\rightarrow t}(S))$ and $(M_i^{t\rightarrow s}(T), M_i^{s\rightarrow t}(M_i^{t\rightarrow s}(T)))$.
 

%The dataset $\gD$ in this setting contains $\bigcup\limits_{i=1}^{2} (S, M_i^{s\rightarrow t}(S)) \cup (M_i^{t\rightarrow s}(T), T)$ 
%, \ie\ $\gD = (S, M_1^{s\rightarrow t}(S)) \cup (M_1^{t\rightarrow s}(T), T)$
%One of the novelty of CBD is cross-translation, where the current level agents must be different from those in previous levels. It is key to our method's success. 
%different variants \emph{multi-agent diversification} (MAD), which does not employ cross-translation, in the WMT En-Fr, En-De and En-Ro tasks. 


From the comparison in \Cref{table:similar_variants}, we see that none of the BD variants noticeably improves the performance across the language pairs, while CBD provides consistent gains of 1.0-2.0 BLEU. In particular, the BD (1{\text{st}} level, 1 agent) variant fails to improve as the distilled model is trained on the same synthetic data that the UMT agent is already trained on. 
The variant BD (1{\text{st}} level, 2 agents) is in fact similar in sprit to \citep{nguyen2019data}, which improves supervised and semi-supervised MT. However, it fails to do so in the unsupervised setup, {due to the lack of supervised agents.}
% This is inspired from data diversification \citep{nguyen2019data}, which improves supervised and semi-supervised MT. 
%\red{any reason why it works in supervised but not in unsupervised? could this be because the same birectional model has been used}\blue{not sure, but it is not because it is bidirectional.} 
% Since the BD (1{\text{st}} level, 2 agents) variant fails, its 2{\text{nd}} level 
The variant BD (2{\text{nd}} level, 2 agents) also fails because the 2{\text{nd}} level synthetic data is already optimized during iterative back-translation training of the UMT agents, leaving the distilled model with no extra information to exploit. On the other hand, cross-model back-translation enables CBD to translate the second-level data by an agent other than the first-level agent. In this strategy, the second agent produces targets that the first agent is not aware of, while the second agent receives as input the sources that are foreign to it. This process creates corrupted but new information, which the supervised MT model can leverage to improve the overall MT performance through more data diversity.

\begin{table}[h!]   
\begin{center}
% \vspace{-1em}
% \resizebox{\columnwidth}{!}{%
\caption{BLEU comparison of CBD vs. no cross-model variants in the WMT'14 English-French (En-Fr), WMT'16 English-German (En-De) and English-Romanian (En-Ro) tasks.
% All experiments are based on the base NMT approach \citep{lample2018phrase_unsup}.
}
\begin{tabular}{lcccccc}
\toprule
{\bf Method}          & {\bf En-Fr} & {\bf Fr-En} & {\bf En-De} & {\bf De-En} & {\bf En-Ro}  & {\bf Ro-En}\\
\midrule
NMT Baseline \citep{lample2018phrase_unsup}   & 24.7	& 24.5  & 14.5	& 18.2	& 16.7	& 16.3    \\
BD   (1${\text{st}}$ level, 1 agent)            & 24.5	& 24.4  & 13.8  & 17.6  & 16.0  & 15.9 \\
BD   (1${\text{st}}$ level, 2 agents)            & 24.6	& 24.6  & 14.0  & 17.9  & 16.5  & 16.1\\
BD   (2${\text{nd}}$ level, 2 agents)            & 24.7	& 24.7  & 14.4  & 18.0  & 16.7  & 16.4\\
CBD  (2${\text{nd}}$ level, 2 agents)            & \textbf{26.5}	& \textbf{25.8}  & \textbf{16.6}	& \textbf{20.4}  & \textbf{18.3}  & \textbf{17.7} \\
\bottomrule
\end{tabular}
% }
\vspace{-1em}
\label{table:similar_variants}
\end{center}
\end{table}


\subsection{CBD produces diverse data} \label{subsec:data_diversity}

% \red{
Having argued that cross-model back-translation creates extra information for the supervised MT model to leverage on, we hypothesize that such extra information can be measurable by the diversity of the generated data. To measure this, we compute the \emph{reconstruction BLEU} and compare the scores for BD and CBD (both 2nd level, 2 agents) in the WMT En-Fr, En-De and En-Ro tasks.
%We measure this by comparing the reconstruction BLEU of MAD and CBD (both 2nd level, $n=2$) in the WMT En-Fr, En-De and En-Ro tasks. 
%(\ie\ BLEU score between the original and the reconstructed texts) 
The scores are obtained by using the first agent to translate the available monolingual data in language $s$ to $t$ and then the second agent to translate those translations back to language $s$. After that, a BLEU score is measured by comparing the reconstructed text with the original text. In BD, the first and second agents are identical, while they are distinct for CBD. From the results in \Cref{table:diversity_bleu}, we observe that the reconstruction BLEU scores of CBD are more than 10 points lower than those of BD, indicating that the newly generated data by CBD are more diverse and different from the original data.
% }
%for $s$-$t$-$s$  between the final outputs to the original data. 

% Table \ref{table:diversity_bleu} shows the reconstruction BLEU scores of MAD and CBD for the WMT En-Fr, En-De and En-Ro tasks. The scores are obtained by using the first agent to translate monolingual data in language $s$ to $t$ and then the second agent to translate those translations back to language $s$. After that, a BLEU score for $s$-$t$-$s$ is measured between the final outputs to the original data. In MAD, the first and second agents are identical, while they are distinct for CBD. As it can be seen, the reconstruction scores of CBD are by more than 10 BLEU lower than that of MAD, indicating that the newly generated data are diverse and different from the original data.

\begin{table}[h!]
\begin{center}
% \vspace{-1em}
% \resizebox{\columnwidth}{!}{%
\caption{Reconstruction BLEU scores of BD and CBD in different languages for the WMT unsupervised translation tasks. Lower BLEU means more diverse.}
\begin{tabular}{lcccccc}
\toprule
% \multirow{2}{*}{\bf Task}   & \multicolumn{4}{c|}{\bf IWSLT} & \multicolumn{2}{c}{\bf WMT-En-De}\\
% \cmidrule{2-7}
{\bf Method }          & {\bf En-Fr-En} & {\bf Fr-En-Fr} & {\bf En-De-En} & {\bf De-En-De} & {\bf En-Ro-En}  & {\bf Ro-En-Ro}\\
\midrule
BD                   & 76.5	& 72.7  & 75.1	& 63.3  & 73.6  & 71.2      \\
CBD                  & 63.1	& 59.5  & 60.7	& 50.6  & 61.0	& 56.8      \\
\bottomrule
\end{tabular}
% }
%\vspace{-1em}
\label{table:diversity_bleu}
\end{center}
\end{table}

%\red{Data diversity can also be measured by the ratio of duplicate source-target pairs to the amount of synthetic parallel data created by  CBD.}\alert{will add BD}
% Table \ref{table:diversity_duplicates} shows the total size of the synthetic parallel data generated CBD and the amount of duplicates for WMT En-Fr, En-De, En-Ro. 



In \Cref{table:diversity_duplicates}, we further report the ratio of duplicate source-target pairs to the amount of synthetic parallel data created by CBD. We sample 30M synthetic parallel data using the CBD strategy and examine the amount of duplicate pairs for the WMT En-Fr, En-De and En-Ro tasks.
% In \Cref{table:diversity_duplicates}, we compare the amount of real data, total synthetic data created by CBD and the amount of duplicate pairs for WMT En-Fr, En-De and En-Ro tasks.
We can notice that across the language pairs, only around 14\% of the parallel data are duplicates. 
% Given that 87.5\% of the data are not real, this amount of duplicates is surprisingly low. 
Given that only about 5M (3.5M for En-Ro) sentences are \emph{real} sentences and the remaining 25M sentences are synthetic, this amount of duplicates is surprisingly low. This fact also explains why CBD is able to exploit extra information better than any standard UMT to improve the performance.
% \todo{The table can be wrapped within text, if we need space}

\begin{table}[h!]
\begin{center}
% \vspace{-1em}
% \resizebox{\columnwidth}{!}{%
\caption{Comparison between the amount of real data, generated data by CBD and the duplicates per language pair for the WMT'14 En-Fr, WMT'16 En-De and En-Ro unsupervised MT tasks.}
\begin{tabular}{lccc}
\toprule
% \multirow{2}{*}{\bf Task}   & \multicolumn{4}{c|}{\bf IWSLT} & \multicolumn{2}{c}{\bf WMT-En-De}\\
% \cmidrule{2-7}
{\bf Method }          & {\bf En-Fr} & {\bf En-De} & {\bf En-Ro} \\
\midrule
% Real data {(monolingual)}              & 5M    & 5M    & 3.5M \\
Real data               & 5M    & 5M    & 3.5M  \\
Generated data          & 30M   & 30M   & 29M   \\
Duplicate pairs         & 4.4M (14.5\%)   & 3.9M(13\%)     & 3.9M (13.4\%) \\
\bottomrule
\end{tabular}
% }
% \vspace{-1em}
\label{table:diversity_duplicates}
\end{center}
\end{table}


%\subsection{CBD outperforms ensembles of models {and ensemble knowledge distillation}}

\subsection{Comparison with ensembles of models {and ensemble knowledge distillation}} \label{subsec:alternatives1}

Since CBD utilizes {outputs from} two UMT agents for supervised distillation, it is interesting to see how  it performs compared to an ensemble of UMT models and ensemble knowledge distillation \citep{ensemble_distill_freitag2017}.
To perform ensembling, we average the probabilities of the two UMT agents at each decoding step. {For ensemble distillation, we generate synthetic parallel data from an ensemble of UMT agents, which is then used to train the supervised model.}


\begin{table}[h!]
\begin{center}
% \vspace{-1em}
% \resizebox{\columnwidth}{!}{%
\caption{BLEU comparison of CBD vs. an ensemble of UMT agents and ensemble knowledge distillation \citep{ensemble_distill_freitag2017} on WMT'14 En-Fr, WMT'16 En-De and En-Ro translation tasks.}
\begin{tabular}{lcccccc}
\toprule
{\bf Method}          & {\bf En-Fr} & {\bf Fr-En} & {\bf En-De} & {\bf De-En} & {\bf En-Ro}  & {\bf Ro-En}\\
\midrule
NMT Baseline {\citep{lample2018phrase_unsup}}                         & 24.7	& 24.5  & 14.5	& 18.2	& 16.7	& 16.3    \\
Ensemble of 2 NMT agents                                            & 25.2	& 24.8	& 15.3	& 19.1	& 17.7	& 17.1 \\
Ensemble distillation       & 17.3	& 20.0 	& 3.5	& 3.7	& 1.2	& 1.1 \\
CBD with NMT               & \textbf{26.5}	& \textbf{25.8}  & \textbf{16.6}	& \textbf{20.4}  & \textbf{18.3}  & \textbf{17.7} \\
\bottomrule
\end{tabular}
% }
\vspace{-1em}
\label{table:compare_with_ensemble}
\end{center}
\end{table}



From the results on the WMT translation tasks in \Cref{table:compare_with_ensemble}, we observe that ensembles of models improve the performance only by 0.5-1.0 BLEU, while CBD provides larger gains (1.0-2.0 BLEU) across all the tasks. 
These results demonstrate that CBD is capable of leveraging the potentials of multiple UMT agents better than how an ensemble of agents does.
This is in contrast to {data diversification} \citep{nguyen2019data}, which is shown to mimic and perform similarly to model ensembling. More importantly, during inference, an ensemble of models requires more memory and computations (twice in this case) to store and execute multiple models. In contrast, CBD can throw away the UMT teacher agents after training and needs only one single model for inference. Meanwhile, ensemble knowledge distillation \citep{ensemble_distill_freitag2017}, which performs well with supervised agents, performs poorly in unsupervised MT tasks. The reason could be that the UMT agents may not be suitable for the method {originally} intended for supervised learning. {Further inspection in {Appendix \Cref{sec:appendix:analysis_duplicates}} suggests that many samples in the ensemble translations contain incomprehensible repetitions.}




\begin{table}[t!]
\begin{center}
% \vspace{-1em}
% \resizebox{\columnwidth}{!}{%
\caption{Comparison with other alternatives on the WMT En-Fr, Fr-En, En-De and De-En, with XLM as the base model.}
\begin{tabular}{lcccc}
    \toprule
    {\bf WMT}              & {\bf En-Fr}    & {\bf Fr-En}  & {\bf En-De} & {\bf De-En} \\
    \midrule
    % Baseline (XLM)                              & 1x & 1x & 33.0	& 31.5  & 23.9  & 29.3  & 30.6   & 27.9 \\
    XLM Baseline {\citep{conneau2019cross_xlm}}                             & 33.0	& 31.5  & 23.9  & 29.3  \\
    \midrule
    Sampling with temperature 0.3                  & 33.5 & 32.2  & 24.3	& 30.2 \\
    Top-k sampling                              & 33.18 & 32.26 & 24.0 & 29.9\\
    Nucleus {(top-p)} sampling                            & \multicolumn{4}{c}{Diverge}\\
    % \midrule
    Target noising                              & 32.8 & 30.7  & 24.0	& 29.6 \\
    Multi-agent dual learning                   & 33.5 & 31.7  & 24.6   & 29.9\\
    % \midrule
    % Train for 8x longer                         & 32.9 & 31.5	& 23.9	& 29.4\\
    % Train with 4x8=32 GPUs                      & 33.6 & 31.7 & 24.0	& 29.5 \\
    % Ensemble of 4/6/8 agents                    & 34/34.2/34.2 & 32.2/32.4/32.5 & 24.8/24.9/25	& 30.4/30.6/30.6 \\
    \midrule
    CBD                                  & 35.3	& 33.0  & 26.1  & 31.5  \\
    \bottomrule
\end{tabular}
% }
\vspace{-1em}
\label{table:compare_with_others}
\end{center}
\end{table}

\subsection{Comparison with other potential alternatives} \label{subsec:alternatives2}

In this section, we compare CBD with other alternatives in the  text generation literature that also attempt to increase diversity. {While many of these methods are generic, we adopt them in the UMT framework and compare their performance with our CBD technique in the WMT En-Fr, Fr-en, En-De, and De-en tasks, taking the XLM \citep{conneau2019cross_xlm} as the base model.} 

One major group of alternatives is \emph{sampling} based methods, where the model samples translations following multinomial distributions during iterative back-translation. Specifically, we compare the CBD with \Ni sampling with temperature 0.3 \citep{understanding_backtranslation_scale,hier_neural_story_gen}, \Nii top-k sampling \citep{radford2019language_gpt2}, and \Niii nucleus or top-p sampling \citep{curious_text_degeneration}. Plus, we compare CBD with \emph{target noising}, where we add random noises to the translations of the UMT model during iterative back-translation. Finally, multi-agent dual learning \citep{multiagent} is also considered as another alternative, where multiple unsupervised agents are used train the end {supervised} model. 
 


The results are reported in \Cref{table:compare_with_others}. We can see that while the sampling based methods indeed increase the diversity significantly, they do not improve the performance as much as CBD does. The reason could be that the extra data generated by {(stochastic)} sampling are noisy and their quality is not as good as deterministic predictions from the two UMT agents via cross-model back-translation. On the other hand, target noising does not provide a consistent improvement while multi-agent dual learning  achieves less impressive gains compared to CBD.


% \vspace{-0.5em}
% & 25.3   & 30.7\\
% \section{Parallel data size and unanswered questions}\label{subsec:questions}
% % explain data growth first, then explain why we didn't do large scale and n=3 or n=4 -> but based on iwslt -> convice that it can improves
% % then look the the tabke horizontally, show that data alsos scaleup with level -> 
% % ? large scale data how?
% % ? n=3 how ?
% % ? 3rd level 4th level

% Even though our CBD method is highly generalizable and scalable, our limited resources have restrained us from conducting very large-scale experiments, thus leaving certain questions unanswered. \Cref{table:data_size} shows the amount of synthetic parallel data that would be generated for different CBD variants for different sizes of monolingual data in each language. A $k$-th level CBD with multiplier $n$ generates a dataset of size $\mathcal{O}(|S|n^k)$, meaning that the required computing power also increases with $n$ and $k$. 
% This would require 1.1B sentence pairs to be translated for the high-resource settings {(137M per-language sentences)} used by \citet{lample2018phrase_unsup} and \citet{conneau2019cross_xlm}. 
% % This would require 1.1B sentence pairs to be translated for the high-resource settings \citep{lample2018phrase_unsup,conneau2019cross_xlm}.
% Thus, we were unable to replicate the large-scale experiments and confirm the effectiveness of CBD in those large-scale settings. Nonetheless, as CBD outperforms the baselines in {5M-sentence} WMT setting (\cref{subsec:wmt}) and {160K-sentence} IWSLT setting (\cref{subsec:iwslt}) across 6 different language pairs {and 8 distinct corpora,} we are confident that it will boost performance for the very large-scale setup as well. 

% Plus, we did not experiment with higher multipliers ($n=3,4$) for the WMT tasks. The ablation study in \cref{subsec:iwslt} indicates that $n=3$ is the best for IWSLT tasks. Thus, it is unclear whether $n=2$, as done in \cref{subsec:wmt}, is the best configuration for the WMT tasks, because a higher multiplier may yield even more gains. Finally, CBD can be scaled up to 3rd, 4th, ... up to $k$-th level. However, we do not include them in the scope of the WMT experiments, due to limited resources. We conjecture that 3rd level CBD causes translation degeneration in the IWSLT tasks (\cref{subsec:iwslt}), but it is uncertain whether it would behave similarly for the much larger datasets in WMT tasks.
% We leave these for future work.

% \begin{table}[h!]
% \begin{center}
% \vspace{-1em}
% % \resizebox{\columnwidth}{!}{%
% \caption{The total size of synthetic parallel dataset produced by the 2nd, 3rd and 4th level CBD with varying multiplier $n$ for monolingual data sizes of 5M (ours) and 137M per language \citep{lample2018phrase_unsup,conneau2019cross_xlm}.}
% \begin{tabular}{cccccccc}
% \toprule
% %\multirow{2}{*}{\bf Multiplier}
% & \multicolumn{3}{c}{\bf $|S|=5M$} & \multicolumn{3}{c}{\bf $|S|= 274M/2 = 137M$} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
%                         & \textbf{$n=2$}    & \textbf{$n=3$}   & \textbf{$n=4$} & \textbf{$n=2$}    & \textbf{$n=3$}   & \textbf{$n=4$} \\
% \midrule
% 2nd level   & 40M	& 90M   & 160M  & 1.1B	& 2.5B  & 4.4B\\
% 3rd level   & -	    & 150M  & 400M  & -	    & 4.1B  & 10.9B \\
% 4th level   & -	    & -     & 640M  & -	    & -     & 17.5B    \\
% \bottomrule
% \end{tabular}
% % }
% \vspace{-1em}
% \label{table:data_size}
% \end{center}
% \end{table}





==> img/Sintro.tex <==



% Machine translation is one of the core tasks in natural language processing (NLP) that involves both language understanding and generation. 
% Advances in machine translation often translate to developments in other fields of NLP, such as representation learning \citep{devlin2018bert,conneau2019cross_xlm,2019t5}, text summarization \citep{rush-etal-2015-neural}, parsing \citep{kitaev-klein-2018-constituency} and dialogue generation \citep{end2end_task_dialogue_li2017end}. 
% Recent neural approaches \citep{vaswani2017attention,payless_wu2018,so2019evolved} achieve the state of the art with near human-level performance \citep{hassanawadalla2018achieving}. However, they continue to rely heavily on large parallel corpora, which are not always available, especially for low-resource languages.

Machine translation (MT) is a core task in natural language processing  that involves both language understanding and generation. Recent neural approaches \citep{vaswani2017attention,payless_wu2018} have advanced the state of the art with near human-level performance \citep{hassanawadalla2018achieving}. 
However, they continue to rely heavily on large parallel data.
% , which are not always available, especially for low-resource languages. 
As a result, the search for unsupervised alternatives using only monolingual data has been active. While \citet{ravi2011deciphering} and \citet{smt_without_parallel_klementiev2012toward} proposed various unsupervised techniques for statistical MT (SMT), \citet{lample2017unsupervised,lample2018phrase_unsup} established a general framework for modern unsupervised MT (UMT) that works for both SMT and neural MT (NMT) models. The framework has three main principles: model initialization, language modeling and iterative back-translation.
Model initialization bootstraps the model with a knowledge prior like word-level transfer \citep{muse_conneau2017word}. Language modeling, which takes the form of denoising auto-encoding (DAE) in NMT \citep{lample2018phrase_unsup}, trains the model to generate plausible sentences in a language. Meanwhile, iterative back-translation (IBT) facilitates cross-lingual translation training by generating noisy source sentences for original target sentences.
The {recent approaches}  differ on how they apply each of these three principles. For instance, \citet{lample2017unsupervised} use an unsupervised word-translation model \citep{muse_conneau2017word} for model initialization, while \citet{conneau2019cross_xlm} use a pretrained cross-lingual masked language model (XLM).
% \todo{Can you cite the conference version of these papers?} 
%\citep{lample2017unsupervised,lample2018phrase_unsup,conneau2019cross_xlm}
%These models express a data-driven prior about how sentences should read in each language, and they improve the quality of the translation models by performing local substitutions and word reorderings.

%\red{While the framework is well-established, there are some discussions on whether there exists a fourth principle that can be a good add-on to the framework.}


% input-side is noised, specific to NMT about what to be said,


{In this paper, we focus on a different aspect of the UMT framework, namely, its \emph{data diversification}\footnote{{By diversification, we mean sentence level variations (not expanding to other topics or genres).}} process. If we look from this view, the DAE and IBT steps of the UMT framework also perform some form of data diversification to train the model.} 
%{In this paper, however, we focus on a different view of the DAE and IBT} steps, that they perform some form of data diversification to train the model. 
Specifically, the noise model in the DAE process generates \emph{new}, but noised, versions of the input data, which are used to train the model with a reconstruction objective. Likewise, the IBT step involves the same
UMT model to create synthetic parallel pairs (with the source being synthetic), which are then used to train the model. Since the NMT model is updated with DAE and IBT simultaneously, the model generates \emph{fresh} translations in each back-translation step. Overall, thanks to DAE and IBT, the model gets better at translating by iteratively training on the newly created and diversified data {whose quality also improves over time.} This argument also applies to statistical UMT, except for the lack of the DAE \citep{lample2018phrase_unsup}. However, we conjecture that these diversification methods may have reached their limit as the performance does not improve further the longer we train the UMT models. 


% this  process may not be the optimal but may \red{face diminishing return}\todo{diminishing return is everywhere and can be a good thing; we need to revise it} as the performance does not improve the longer we train the UMT model.

%processes do not progress %forever, but may face diminishing return as the performance does not improve the longer we train the UMT model.




%In this paper, however, we view the denoising auto-encoding (only for NMT) and iterative back-translation steps as forms of data diversification to train the UMT model. 

%As the original model gets better at translating, we use the current model to improve the back-translation model, resulting in a coupled system trained with an iterative algorithm

% for NMT, the denoising auto-encoding step randomly and constantly generates \emph{new}, but noised, versions of the data, which are used as input to train the model with a reconstruction objective. Likewise, the iterative back-translation step involves the same UMT model translating the monolingual data to create synthetic parallel pairs (with the input-side being synthetic), which are then used to train the model. 

%Since the NMT model is updated with DAE and IBT simultaneously,  the UMT model generates \emph{fresh} translations during each back-translation step. Overall, thanks to denoising auto-encoding and iterative back-translation, the model is iteratively trained on newly created and diversified data that are gradually improving in quality. This argument also applies for SMT, except for the lack of DAE. However, we conjecture that these diversification processes do not progress forever, but may face diminishing return as the performance does not improve the longer we train the UMT model.

In this work, we introduce a fourth principle to the standard UMT framework: Cross-model Back-translated Distillation or CBD (\cref{sec:method}), with the aim to induce another level of diversification that the existing UMT principles lack.  CBD initially trains two UMT agents (models) using existing approaches. Then, one of the two agents translates the monolingual data from one language $s$ to another $t$ in the first level. In the second level, the generated data are back-translated from $t$ to $s$ by the \emph{other agent}. In the final step, the synthetic parallel data created by the first and second levels are used to distill a supervised MT model. CBD is applicable to any existing UMT method {and is more efficient than ensembling approaches \citep{ensemble_distill_freitag2017}} (\cref{subsec:alternatives1}). 

%and is shown in this paper to significantly improve the performance of the underlying UMT methods.

%another component to the common unsupervised MT framework: Cross-model Back-translated Distillation (CBD). The technique is applicable to any existing UMT methods and is shown in this paper to significantly improve the performance of the underlying UMT method. The procedure first trains two (2) UMT agents (models) using existing approaches. Then, one of agents translates the monolingual data from one language $s$ to another $t$ in the first level. After that, in the second level, the generated data are then back-translated from $t$ back $s$ by the \emph{the other agent}. In the final step, the synthetic parallel data created by the first and second level are used to distill a supervised MT model.


%While the UMT framework is a well-established one, we propose to extend it to include a fourth principle that we propose in this work for further improvements. In particular, 


% This paper introduces a new add-on to the three-principle UMT framework: Multi-Agent Cross-Translated Diversification (MACD). The technique is applicable to any existing UMT methods and is shown in this paper to significantly improve the performance of the underlying UMT method. The procedure first trains multiple UMT agents (models), then each of them translates the monolingual data from one language $X$ to another $Y$ in the first level. After that, in the second level, the generated data are again translated from language $Y$ back to $X$ by agents other than the one of its origin to produce level 2 synthetic data - a process which we call \emph{cross-translation}. The process continues until the $k$-th level. In the final step, a supervised MT model is trained on all those synthetic parallel data. 


In the experiments (\cref{sec:experiments}), we have evaluated CBD on the WMT'14 English-French, WMT'16 English-German and WMT'16 English-Romanian unsupervised translation tasks. 
% \red{We compare our results against the existing UMT methods, such as the unsupervised NMT and Phrase based SMT (PBSMT)  proposed by \citet{lample2018phrase_unsup} and the model with a pretrained  XLM \citep{conneau2019cross_xlm}.}\todo{I'd exclude this} 
CBD shows consistent improvements of 1.0-2.0 BLEU compared to the baselines in these tasks. It also boosts the performance on IWSLT'14 English-German and IWSLT'13 English-French tasks {significantly}. {In our analysis, we explain with experiments why other similar variants (\cref{subsec:cross_translation}) {and other alternatives from the literature (\cref{subsec:alternatives2})} do not work well and cross-model back-translation is crucial for our method.} We further demonstrate that CBD enhances the baselines by achieving greater diversity as measured by back-translation BLEU (\cref{subsec:data_diversity}). 
% \red{add low-resource later}


\begin{comment}

\citep{pbsmt_Koehn:2003:SPT}

\citep{vaswani2017attention}
\citep{payless_wu2018}
\citep{sennrich2015neural}
\citep{luong2015effective}
\citep{muse_conneau2017word}
\citep{nguyen2019data}
\citep{knowledge_distill_kim_rush_2016}
\citep{kim2016sequence_knowledge_distillation}
\citep{denoising_ae_vincent2008extracting}
\citep{ensemble_distill_freitag2017}
\citep{effectove-artetxe-etal-2019}
\citep{devlin2018bert}
\citep{lample2017unsupervised}
\citep{lample2018phrase_unsup}
\citep{conneau2019cross_xlm}

\end{comment}


==> img/Smethod.tex <==
% \section{Multi-agent cross-translated diversification}

\section{Cross-model Back-translated Distillation} \label{sec:method}
Let $\sX_{s}$ and $\sX_{t}$ be the sets of monolingual data for languages $s$ and $t$, respectively. We first train two UMT agents independently with two different parameter sets $\theta_1$ and $\theta_2$ using existing methods \citep{lample2017unsupervised,lample2018phrase_unsup,conneau2019cross_xlm}.\footnote{For neural approaches, changing the random seeds would do the trick, while PBSMT methods would need to randomize the initial embeddings and/or subsample the training data.} Since a UMT agent with parameter set $\theta$ is deemed bidirectional in our setup, we denote $y_t \sim P(\cdot|x_s,\theta)$ to be the translation sample from language $s$ to $t$ of input sentence $x_s$ using parameters $\theta$. In addition, for each language direction $s\rightarrow t$ (and vice versa for $t\rightarrow s$), we introduce a \emph{supervised} MT model with parameters $\hat{\theta}$ that will be trained through our CBD. With these notations, we denote the following training loss $\mathcal{L}$ with respect to input variables $\theta_{\alpha}$, $\theta_{\beta} \in \{\theta_1,\theta_2\}$, the supervised parameters $\hat{\theta}$ and the learning rate $\eta$. \Cref{fig:cbd:translation_diagram} also illustrates the translation flows of function $\mathcal{L}$.
\begin{equation}
\begin{aligned}
\mathcal{L}(\theta_{\alpha},\theta_{\beta}, \hat{\theta}) &= -\E_{z_s \sim P(\cdot|y_t,\theta_{\beta}), y_t \sim P(\cdot|x_s,\theta_{\alpha}), x_s \sim \sX_s} \big[ \log P(y_t|x_s,\hat{\theta}) + \log P(y_t|z_s,\hat{\theta}) \big] \\
    &\quad -\E_{z_t \sim P(\cdot|y_s,\theta_{\beta}), y_s \sim P(\cdot|x_t, \theta_{\alpha}), x_t \sim \sX_t} \big[ \log P(x_t|y_s,\hat{\theta}) + \log P(z_t|y_s,\hat{\theta}) \big]
\end{aligned}
\label{eqn:cbd_loss}
\end{equation}
In the CBD strategy (\Cref{alg:macd}, Eq. \ref{eqn:cbd_loss}), at each step, each agent $\theta \in \{\theta_1,\theta_2\}$ samples {translations} from the monolingual data of both languages $s$ and $t$ to acquire the \emph{first level} of synthetic parallel data $(x_s$,$y_t)$ and $(x_t$,$y_s)$. In the \emph{second level}, the other agent $\{\theta_1,\theta_2\} \setminus \theta$ is used to sample the translation $z_s$ of the translation $y_t$ of $x_s$ (and similarly for $z_t$ from the translation $y_s$ of $x_t$). This process is basically back-translation, but with the backward model coming from a different regime than that of the forward model. The fact that the first level agent must be different from the second level agent is crucial to achieve the desirable level of diversity in data generation. After this, we update the final model $\hat{\theta}$ using {all the} synthetic pairs $(x,y)$ and $(y,z)$ with maximum likelihood estimation (MLE).

% In this section, we describe the MACD procedure in detail. Let $S$ and $T$ be the sets of monolingual data for languages $l_1$ and $l_2$, respectively. We first train $n$ UMT agents $M_1,M_2,...,M_n$, where $n$ is called the \emph{diversification multiplier}. The agents can be implemented following any of the existing UMT techniques \citep{lample2017unsupervised,lample2018phrase_unsup,conneau2019cross_xlm}. They are trained independently and randomly such that no two agents are the same or guaranteed to generate the same output for any given input.\footnote{For neural approaches, changing the random seeds would do the trick, while PBSMT methods would need to randomize the initial embeddings and/or subsample the training data.} Because a UMT agent $M_i$ is deemed bidirectional in our setup, we denote $M_i^{s\rightarrow t}(X_s)=Y$ to be the translations from language $s$ to $t$ of corpus $X_s$ (of language $s$) by UMT agent $M_i$, and vice versa for $M_i^{t\rightarrow s}(X_t)=Y$. The translations can be performed using standard greedy search or beam search. 

%In this section, we describe the CBD procedure in details. 

%Since a UMT agent with parameter set $\theta$ is deemed bidirectional in our setup, we denote $y \sim P(\cdot|x,\theta,s,t)$ to be the translation sample from language $s$ to $t$ of input sentence $x$ (in language $s$) using parameters $\theta$. In addition, for each language direction $s\rightarrow t$ (and vice versa for $t\rightarrow s$), we introduce a \emph{supervised} MT model with parameters $\hat{\theta}$ that will be trained through CBD. 


%With these notations, we denote the training loss $\mathcal{L}$ with respective to input variable $\theta_{\alpha}$, $\theta_{\beta}$, language $s$, $t$ and supervised parameter $\hat{\theta}$ as follow:


\begin{comment}
\begin{equation}
\begin{aligned}
\mathcal{L}(\theta_{\alpha},\theta_{\beta}, s, t, \hat{\theta}) &= -\E_{z\sim P(\cdot|y,\theta_{\beta},t,s),y\sim P(\cdot|x,\theta_{\alpha},s,t),x\sim X_s} (\log P(y|x,\hat{\theta}) + \log P(y|z,\hat{\theta}))\\
    &\quad -\E_{z\sim P(\cdot|y,\theta_{\beta},t,s),y\sim P(\cdot|x,\theta_{\alpha},t,s),x\sim X_t} (\log P(x|y,\hat{\theta}) + \log P(z|y,\hat{\theta}))
\end{aligned}
\label{eqn:cbd_loss}
\end{equation}
\end{comment}


% In this section, we first formally describe our data diversification strategy (\cref{subsec:datadiver}), then we  compare it with other related methods in the literature (\cref{subsec:rel}).  

% \subsection{Two-Stage Data Diversification} \label{subsec:datadiver}
    
    % Let $\gD = (S, T)$ be the parallel training data, where $S$ denotes the source-side corpus and $T$ denotes the target-side corpus. Also, {let $M_{S \rightarrow T}$ and $M_{T \rightarrow S}$} be the forward and backward NMT models, which translate from source to target and from target to source, respectively. In our case, we use the Transformer \citep{vaswani2017attention} as the base architecture. In addition, given a corpus $X_l$ in language $l$ and an NMT model $M_{l \rightarrow \hat{l}}$ which translates from language $l$ to language $\hat{l}$, we denote the corpus $M_{l \rightarrow \hat{l}}(X_l)$ as the translation of corpus $X_l$ produced by the model $M_{l \rightarrow \hat{l}}$. The translation may be conducted following the standard procedures such as maximum likelihood and beam search inference.
    
    % % training with cross entropy loss

% ----- This version present the generalized version

% \begin{algorithm}[t!]
% % \caption{Positional Encoded Up-sampling: given an image feature map $M$ which has $D$ dimensions resolution $S$ and $C$ channels, return up-sampled image feature map $M'$ that has resolution $2S$}
% %\small
% \footnotesize
% \caption{$k$-{\text{th}} level MACD: Given monolingual data $S$ and $T$, a diversification multiplier $n$ and level $k$ where $n \geq k$; return trained source-target and target-source MT models $\hat{M}_{s \rightarrow t}$ and $\hat{M}_{t \rightarrow s}$.}
% % \label{alg:macd_klevel}
% \label{alg:macd}
% \begin{algorithmic}[1]
% \Procedure{TrainUnsup}{$S,T$}
%     % \State Initialize $M$ with random parameters $\theta$
%     \State Train randomly initialized $M$ on $S\cup T$ until convergence with \textbf{unsupervised} method.
%     \State \textbf{return} $M$
% \EndProcedure
% \end{algorithmic}
% \begin{algorithmic}[1]
% \Procedure{TrainSup}{$\gD = (S,T)$}
%     % \State Initialize $M$ with random parameters $\theta$
%     \State Train randomly initialized $M$ on $\gD = (S,T)$ until convergence with \textbf{supervised} method.
%     \State \textbf{return} $M$
% \EndProcedure
% \end{algorithmic}
% \begin{algorithmic}[1]
% \Procedure{Reverse}{$\gD = (S,T)$}
%     % \State Initialize $M$ with random parameters $\theta$
%     \State \textbf{return} $\gD' = (T,S)$ \algorithmiccomment{Reverse the parallel data}
% \EndProcedure
% \end{algorithmic}
% \begin{algorithmic}[1]
% \Procedure{Recur\_MACD}{$\mathcal{M}, \mathcal{U}, n, k, S, T$}
%     \State \textbf{if} $k=0$ \textbf{then return} $ (\varnothing, \varnothing)$
%     \State $\gD \gets (\varnothing, \varnothing)$ \algorithmiccomment{Initialize pseudo-parallel dataset}
%     \For{$M_j \in \mathcal{M}$ where $M_j \not\in \mathcal{U}$}
%         \State $\gD \gets \gD \cup (S, M_j^{s\rightarrow t}(S)) $  \algorithmiccomment{Add synthetic data built from source}
%         \State $\gD \gets \gD \cup (M_j^{t\rightarrow s}(T), T)$ \algorithmiccomment{Add synthetic data built from target}
%         \State Push $M_j$ into $\mathcal{U}$
%         \State $\gD \gets \gD \cup \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k - 1, M_j^{t\rightarrow s}(T), M_j^{s\rightarrow t}(S))$
%         \State Pop $M_j$ out of $\mathcal{U}$
%     \EndFor
%     \State \textbf{return} $\gD$
% \EndProcedure
% \end{algorithmic}
% \begin{algorithmic}[1]
% \Procedure{General\_MACD}{$S,T,n,k$}
%     \State $\mathcal{M} \gets \varnothing$ \algorithmiccomment{Set of UMT agents}
%     \For{$i \in 1, \ldots,n$}
%         \State $M_i \gets \textsc{TrainUnsup}(S,T)$ \algorithmiccomment{Train UMT agent}
%         \State $\mathcal{M} \gets \mathcal{M}\cup \{M_i\}$
%     \EndFor
%     % \State $\gD \gets (\varnothing, \varnothing)$ \algorithmiccomment{Initialize pseudo-parallel dataset}
%     \State $\mathcal{U} \gets \text{Empty LIFO stack}$ \algorithmiccomment{Initialize agent stack}
%     % \State $\gD \gets \gD \cup \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k, M_i^{t\rightarrow s}(T), M_i^{s\rightarrow t}(S))$
%     \State $\gD \gets \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k, S, T)$ \algorithmiccomment{Generate synthetic parallel data}
%     \State $\hat{M}_{s \rightarrow t} \gets \textsc{TrainSup}(\gD)$  \algorithmiccomment{Train the final model for $s\rightarrow t$}
%     \State $\hat{M}_{t \rightarrow s} \gets \textsc{TrainSup}(\gD'=\textsc{Reverse}(\gD))$  \algorithmiccomment{Train the final model for $t\rightarrow s$}
%     \State \textbf{return} $\hat{M}_{s \rightarrow t}$, $\hat{M}_{t \rightarrow s}$
% \EndProcedure
% \end{algorithmic}
% % \vspace{-1em}
% \end{algorithm}


% \begin{algorithm}[t!]
% \footnotesize
% \caption{Cross-model Back-translated Distillation: Given monolingual data $\sX_{s}$ and $\sX_{t}$ of languages $s$ and $t$, return a $s\rightarrow t$ UMT model with parameters $\hat{\theta}$.}
% \label{alg:macd}
% \begin{algorithmic}[1]
% \Procedure{CBD}{$s,t$}
%     \State Train the 1st UMT agent with parameters $\theta_1$
%     \State Train the 2nd UMT agent with parameters $\theta_2$
%     \State Randomly initialize the parameters for the supervised MT model, $\hat{\theta}$
%     \While{until convergence}
%         \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_1,\theta_2, \hat{\theta})$
%         \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_2,\theta_1, \hat{\theta})$
%     \EndWhile
%     \State \textbf{return} $\hat{\theta}$
% \EndProcedure
% \end{algorithmic}
% % \vspace{-1em}
% \end{algorithm}

    
    % % \begin{columns}[T] % align columns
    % % \begin{column}{.48\textwidth}
\begin{minipage}{\textwidth}
\vspace{-1em}
\begin{minipage}[b]{0.58\textwidth}
\centering
% \resizebox{\columnwidth}{!}{%
% \setlength\tabcolsep{2pt}
\begin{algorithm}[H]
\footnotesize
\caption{Cross-model Back-translated Distillation: Given monolingual data $\sX_{s}$ and $\sX_{t}$ of languages $s$ and $t$, return a $s\rightarrow t$ UMT model with parameters $\hat{\theta}$.}
\label{alg:macd}
\begin{algorithmic}[1]
\Procedure{CBD}{$s,t$}
    \State Train the 1st UMT agent with parameters $\theta_1$
    \State Train the 2nd UMT agent with parameters $\theta_2$
    \State Randomly initialize the parameters for MT model, $\hat{\theta}$
    \While{until convergence}
        \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_1,\theta_2, \hat{\theta})$
        \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_2,\theta_1, \hat{\theta})$
    \EndWhile
    \State \textbf{return} $\hat{\theta}$
\EndProcedure
\end{algorithmic}
% \vspace{-1em}
\end{algorithm}
% \setlength\tabcolsep{6pt}
% }
\vspace{-0.5em}
% \captionof{table}{left caption.}
% \label{table:classification}
\end{minipage}
\hfill
\begin{minipage}[b]{0.40\textwidth}
% \end{column}%
% \hfill%
% \begin{column}{.48\textwidth}
\centering
% \setlength\tabcolsep{2pt}
\begin{figure}[H]
% \begin{equation*}
%     X_s \dashrightarrow x_s  \xrightarrow[s \rightarrow t]{\theta_{\alpha}}  y_t \xrightarrow[t \rightarrow s]{\theta_{\beta}} z_s
% \end{equation*}
% \begin{equation*}
%     X_t \dashrightarrow x_t  \xrightarrow[t \rightarrow s]{\theta_{\alpha}}  y_s \xrightarrow[s \rightarrow t]{\theta_{\beta}} z_t
% \end{equation*}
\begin{equation*}
    X_s \dashrightarrow x_s  \xrightarrow[s \rightarrow t]{\theta_{\alpha}}  y_t \xrightarrow[t \rightarrow s]{\theta_{\beta}} z_s \xRightarrow[(z_s,y_t)]{(x_s,y_t)} \hat{\theta}
\end{equation*}
\begin{equation*}
    X_t \dashrightarrow x_t  \xrightarrow[t \rightarrow s]{\theta_{\alpha}}  y_s \xrightarrow[s \rightarrow t]{\theta_{\beta}} z_t \xRightarrow[(y_s,z_t)]{(y_s,x_t)} \hat{\theta}
\end{equation*}
\caption{Translation flows of loss function $\mathcal{L}$ in Eq. \ref{eqn:cbd_loss}. Variable set $(\theta_{\alpha},\theta_{\beta})$ is replaced with $(\theta_1,\theta_2)$ and $(\theta_2,\theta_1)$ iteratively in \Cref{alg:macd}. Parallel pairs $(x_s,y_t)$,$(z_s,y_t)$,$(y_s,x_t)$ and $(y_s,z_t)$ are used to train the final model $\hat{\theta}$.}
\label{fig:cbd:translation_diagram} 
\end{figure}
% \begin{equation}
%     X_s \rightarrow x_s  \xrightarrow[s \rightarrow t]{\theta_1}  y_t \xrightarrow[t \rightarrow s]{\theta_2} z_t
% \end{equation}
% \begin{equation}
%     X_t \rightarrow x_t  \xrightarrow[t \rightarrow s]{\theta_1}  y_s \xrightarrow[s \rightarrow t]{\theta_2} z_t
% \end{equation}
% \begin{equation}
%     X_s \rightarrow x_s  \xrightarrow[s \rightarrow t]{\theta_2}  y_t \xrightarrow[t \rightarrow s]{\theta_1} z_t
% \end{equation}
% \begin{equation}
%     X_t \rightarrow x_t  \xrightarrow[t \rightarrow s]{\theta_2}  y_s \xrightarrow[s \rightarrow t]{\theta_1} z_t
% \end{equation}
% \setlength\tabcolsep{6pt}
\vspace{-0.5em}
\end{minipage}
\end{minipage}
% \end{column}%
% \end{columns}


% \captionsetup[subfigure]{labelformat=empty}



% \begin{figure}
% % \centering
% % \vspace{-1em}
% \begin{center}
% \begin{subfigure}{.48\textwidth}
%   \begin{center}
%     % \begin{algorithm}[t!]
%     \begin{algorithm}[H]
%     \footnotesize
%     % \ContinuedFloat
%     % \caption*{Part 2}
%     % \caption*{Cross-model Back-translated Distillation: Given monolingual data $\sX_{s}$ and $\sX_{t}$ of languages $s$ and $t$, return a $s\rightarrow t$ UMT model with parameters $\hat{\theta}$.}
%     \captionof{algorithm}{caption text}
%     \label{alg:macd2}
%     \begin{algorithmic}[1]
%     \Procedure{CBD}{$s,t$}
%         \State Train the 1st UMT agent with parameters $\theta_1$
%         \State Train the 2nd UMT agent with parameters $\theta_2$
%         \State Randomly initialize MT parameters $\hat{\theta}$
%         \While{until convergence}
%             \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_1,\theta_2, \hat{\theta})$
%             \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_2,\theta_1, \hat{\theta})$
%         \EndWhile
%         \State \textbf{return} $\hat{\theta}$
%     \EndProcedure
%     \end{algorithmic}
%     % \vspace{-1em}
%     \end{algorithm}
%   \end{center}
% \end{subfigure}
% \hspace{1em}
% \begin{subfigure}{.48\textwidth}
%   \begin{center}
%     \begin{equation}
%     X_s \rightarrow x_s  \xrightarrow[s \rightarrow t]{\theta_{\alpha}}  y_t \xrightarrow[t \rightarrow s]{\theta_{\beta}} z_s
% \end{equation}
% \begin{equation}
%     X_t \rightarrow x_t  \xrightarrow[t \rightarrow s]{\theta_{\alpha}}  y_s \xrightarrow[s \rightarrow t]{\theta_{\beta}} z_t
% \end{equation}
%   \end{center}
% \end{subfigure}%
% \end{center}
% % \vspace{-1em}
% % \caption{Training data size and training/inference time analysis.}
% \label{fig:exp:time_portion}
% %\vspace{-1em}
% \end{figure}





% \ref{algo:macd_general}
% The MACD strategy can be generalized to the $k^{\text{th}}$ level. However, for the sake of brevity and the scope of our experiments, we only describe the second level variant in this paper. We provide a recursive algorithm and other details for the $k^{\text{th}}$ level generalized MACD in the Appendix. 
%$s\rightarrow t$ 

% \alert{Rename cross-translation to something else, and rename MACD}



%In the CBD strategy (\Cref{alg:macd}), at each step, each agent $\theta \in \{\theta_1,\theta_2\}$ samples translations from the monolingual data of both languages $s$ and $t$ to acquire the \emph{first level} of synthetic parallel data $y$. In the second level, the other agent $\Theta \setminus \theta$ is used to sample the translation $z$ of the translation $y$ of $x$. This process is basically back-translation, but with the backward model coming from a different regime than that of the forward model. The fact that the first level agent must be different from the second level agent is crucial to achieve desirable level of diversity in data generation. After this, we update the final model $\hat{\theta}$ with synthetic pairs $(x,y)$ and $(y,z)$ with maximum likelihood estimation (MLE).\todo{The process can be shown as a data flow for better understanding.}

In this way, the model $\hat{\theta}$ first gets trained on the translated products ($x-y$) of the UMT teachers, making it as capable as the teachers. Secondly, the model $\hat{\theta}$ is also trained on the second-level data ($y-z$), which is slightly different from the first-level data. Thus, this mechanism provides extra data diversification to the system $\hat{\theta}$ in addition to what the UMT teachers already offer, resulting in our final model outperforming the UMT baselines (\cref{sec:experiments}). However, one may argue that since $\theta_1$ and $\theta_2$ are trained in a similar fashion, $z$ will be the same as $x$, resulting in a duplicate pair. In our experiments, on the contrary, the back-translated dataset contains only around 14\% duplicates across different language pairs, as shown in our analysis on data diversity in \cref{subsec:data_diversity}.%\todo{I have a suggestion for Figure 1.} 
In Appendix \Cref{sec:appendix:generalized_version}, we provide a more generalized version of CBD with $n$ ($\ge2$) UMT agents, where we also analyze its effectiveness on the IWSLT translation tasks.


% The MACD strategy (\Cref{alg:macd}) first sets up an empty \emph{supervised} dataset, $\gD=(\varnothing, \varnothing)$. Then, each agent $M_i$ performs translations from the monolingual data of both sides $S$ and $T$ to acquire synthetic parallel data $(S, M_i^{s\rightarrow t}(S))$ and $(M_i^{t\rightarrow s}(T), T)$, which are then added to $\gD$. Since at this stage only one UMT agent is used to generate the synthetic dataset, this stage is defined as the first level of diversification. In the second level, for each agent $M_i$, another agent $M_j$ ($M_i \neq M_j$) is deployed to translate the \emph{translations} by $M_i$ back to the original language. This process is basically {back-translation}, but with the backward model $M_j$ coming from a different regime than that of the forward model $M_i$. The fact that $M_j$ must be different from $M_i$ is {indeed crucial to achieve diversity in data generation} and the reason why our method is called ``cross-translated''. We then add this second level of synthetic parallel data (which no longer contain the real monolingual data) to the dataset $\gD$. More specifically, in the second level, dataset $\gD$ is appended with $(M_j^{t\rightarrow s}(M_i^{s\rightarrow t}(S)), M_i^{s\rightarrow t}(S))$ and $(M_i^{t\rightarrow s}(T), M_j^{s\rightarrow t}(M_i^{t\rightarrow s}(T)))$. The process goes on where the agents at the $k$-{\text{th}} level translate the products of their counterparts at level $k-1$. In the final step, we train a newly supervised MT model on this augmented data. Algorithm \ref{alg:macd} outlines the entire process of MACD.     

  %those synthetic parallel data, which now no longer contain the real monolingual data, to the dataset $\gD$. 
  
      %$(k-1)^{\text{th}}$ level counterparts. 
      
% \ie\
% It is worth noting that the total size of the synthetic parallel data grows quadratically with regard to the multiplier $n$ in second level MACD, cubically in the third level, and so on. More accurately, assuming the sizes of monolingual data $S$ and $T$ are equal (\textit{i.e.,} $|S|=|T|$), the total data size $|\gD|$ is:
% \begin{equation}
%     |\gD| = |S|\left( 2\sum_{i=1}^k \Myperm{k} \right) = 2|S| \sum_{i=1}^k \frac{n!}{(n-k)!} \label{eqn:data_size}
% \end{equation}
%where $P(n,k)$ is the $k$-permutations of $n$. 

% \red{On one hand, this is favourable for a supervised NMT model which is inherently data hungry and performs well on very large dataset. Nonetheless, one may argue that such model only performs well on a dataset with minimal duplicates, whereas $\gD$ is prone to be overwhelmed with duplicates because there is no additional real data sources and the UMT agents just translate the monolingual data back and forth. In our experiments, on the contrary, the dataset $\gD$ contains only around 14\% duplicates across different language pairs. We show our analysis on data diversity in Section \ref{subsec:data_diversity}.
% }

% ---------------------------------------------------------------------------------------
    % \section{Multi-agent cross-translated diversification}
    
    % % In this section, we describe the MACD procedure in detail. Let $S$ and $T$ be the sets of monolingual data for languages $l_1$ and $l_2$, respectively. We first train $n$ UMT agents $M_1,M_2,...,M_n$, where $n$ is called the \emph{diversification multiplier}. The agents can be implemented following any of the existing UMT techniques \citep{lample2017unsupervised,lample2018phrase_unsup,conneau2019cross_xlm}. They are trained independently and randomly such that no two agents are the same or guaranteed to generate the same output for any given input.\footnote{For neural approaches, changing the random seeds would do the trick, while PBSMT methods would need to randomize the initial embeddings and/or subsample the training data.} Because a UMT agent $M_i$ is deemed bidirectional in our setup, we denote $M_i^{s\rightarrow t}(X_s)=Y$ to be the translations from language $s$ to $t$ of corpus $X_s$ (of language $s$) by UMT agent $M_i$, and vice versa for $M_i^{t\rightarrow s}(X_t)=Y$. The translations can be performed using standard greedy search or beam search. 
    
    % In this section, we describe the MACD procedure in details. Let $X_{l_1}$ and $X_{l_2}$ be the sets of monolingual data for languages $l_1$ and $l_2$, respectively. We firs train two UMT agents independently with two different parameters $\theta_1$ and $\theta_2$ using existing methods \citep{lample2017unsupervised,lample2018phrase_unsup,conneau2019cross_xlm}.\footnote{For neural approaches, changing the random seeds would do the trick, while PBSMT methods would need to randomize the initial embeddings and/or subsample the training data.} Since a UMT agent with parameter $\theta$ is deemed bidirectional in our setup, we denote $y \sim P(\cdot|x,\theta,s,t)$ to be the translation sample from language $s$ to $t$ of input sentence $x$ (of language $s$) using parameter $\theta$.
    
    % % \begin{equation}
    % %     \mathcal{L}_{f}(\theta, s, t, \hat{\theta}) = -\E_{y \sim P(\cdot|x,\theta,s,t),x \sim X_s} \log P(y|x,\hat{\theta},s,t) - \E_{y \sim P(\cdot|x,\theta,t,s),x \sim X_t} \log P(x|y,\hat{\theta},s,t)
    % % \end{equation}
    
    % % \begin{equation}
    % %     \mathcal{L}_{b}(\theta_{\alpha},\theta_{\beta}, s, t, \hat{\theta}) = -\E_{y \sim P(\cdot|x,\theta,s,t),x \sim X_s} \log P(y|x,\hat{\theta},s,t) - \E_{y \sim P(\cdot|x,\theta,t,s),x \sim X_t} \log P(x|y,\hat{\theta},s,t)
    % % \end{equation}
    
    % \begin{equation}
    % \begin{aligned}
    % \mathcal{L}(\theta_{\alpha},\theta_{\beta}, s, t, \hat{\theta}) &= -\E_{z\sim P(\cdot|y,\theta_{\beta},t,s),y\sim P(\cdot|x,\theta_{\alpha},s,t),x\sim X_s} (\log P(y|x,\hat{\theta}) + \log P(y|z,\hat{\theta}))\\
    %     &\quad -\E_{z\sim P(\cdot|y,\theta_{\beta},t,s),y\sim P(\cdot|x,\theta_{\alpha},t,s),x\sim X_t} (\log P(x|y,\hat{\theta}) + \log P(z|y,\hat{\theta}))\\
    % \end{aligned}
    % \end{equation}
    
    
    % % In this section, we first formally describe our data diversification strategy (\cref{subsec:datadiver}), then we  compare it with other related methods in the literature (\cref{subsec:rel}).  
    
    % % \subsection{Two-Stage Data Diversification} \label{subsec:datadiver}
        
    %     % Let $\gD = (S, T)$ be the parallel training data, where $S$ denotes the source-side corpus and $T$ denotes the target-side corpus. Also, {let $M_{S \rightarrow T}$ and $M_{T \rightarrow S}$} be the forward and backward NMT models, which translate from source to target and from target to source, respectively. In our case, we use the Transformer \citep{vaswani2017attention} as the base architecture. In addition, given a corpus $X_l$ in language $l$ and an NMT model $M_{l \rightarrow \hat{l}}$ which translates from language $l$ to language $\hat{l}$, we denote the corpus $M_{l \rightarrow \hat{l}}(X_l)$ as the translation of corpus $X_l$ produced by the model $M_{l \rightarrow \hat{l}}$. The translation may be conducted following the standard procedures such as maximum likelihood and beam search inference.
        
    %     % % training with cross entropy loss
    
    % % ----- This version present the generalized version
    
    % % \begin{algorithm}[t!]
    % % % \caption{Positional Encoded Up-sampling: given an image feature map $M$ which has $D$ dimensions resolution $S$ and $C$ channels, return up-sampled image feature map $M'$ that has resolution $2S$}
    % % %\small
    % % \footnotesize
    % % \caption{$k$-{\text{th}} level MACD: Given monolingual data $S$ and $T$, a diversification multiplier $n$ and level $k$ where $n \geq k$; return trained source-target and target-source MT models $\hat{M}_{s \rightarrow t}$ and $\hat{M}_{t \rightarrow s}$.}
    % % % \label{alg:macd_klevel}
    % % \label{alg:macd}
    % % \begin{algorithmic}[1]
    % % \Procedure{TrainUnsup}{$S,T$}
    % %     % \State Initialize $M$ with random parameters $\theta$
    % %     \State Train randomly initialized $M$ on $S\cup T$ until convergence with \textbf{unsupervised} method.
    % %     \State \textbf{return} $M$
    % % \EndProcedure
    % % \end{algorithmic}
    % % \begin{algorithmic}[1]
    % % \Procedure{TrainSup}{$\gD = (S,T)$}
    % %     % \State Initialize $M$ with random parameters $\theta$
    % %     \State Train randomly initialized $M$ on $\gD = (S,T)$ until convergence with \textbf{supervised} method.
    % %     \State \textbf{return} $M$
    % % \EndProcedure
    % % \end{algorithmic}
    % % \begin{algorithmic}[1]
    % % \Procedure{Reverse}{$\gD = (S,T)$}
    % %     % \State Initialize $M$ with random parameters $\theta$
    % %     \State \textbf{return} $\gD' = (T,S)$ \algorithmiccomment{Reverse the parallel data}
    % % \EndProcedure
    % % \end{algorithmic}
    % % \begin{algorithmic}[1]
    % % \Procedure{Recur\_MACD}{$\mathcal{M}, \mathcal{U}, n, k, S, T$}
    % %     \State \textbf{if} $k=0$ \textbf{then return} $ (\varnothing, \varnothing)$
    % %     \State $\gD \gets (\varnothing, \varnothing)$ \algorithmiccomment{Initialize pseudo-parallel dataset}
    % %     \For{$M_j \in \mathcal{M}$ where $M_j \not\in \mathcal{U}$}
    % %         \State $\gD \gets \gD \cup (S, M_j^{s\rightarrow t}(S)) $  \algorithmiccomment{Add synthetic data built from source}
    % %         \State $\gD \gets \gD \cup (M_j^{t\rightarrow s}(T), T)$ \algorithmiccomment{Add synthetic data built from target}
    % %         \State Push $M_j$ into $\mathcal{U}$
    % %         \State $\gD \gets \gD \cup \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k - 1, M_j^{t\rightarrow s}(T), M_j^{s\rightarrow t}(S))$
    % %         \State Pop $M_j$ out of $\mathcal{U}$
    % %     \EndFor
    % %     \State \textbf{return} $\gD$
    % % \EndProcedure
    % % \end{algorithmic}
    % % \begin{algorithmic}[1]
    % % \Procedure{General\_MACD}{$S,T,n,k$}
    % %     \State $\mathcal{M} \gets \varnothing$ \algorithmiccomment{Set of UMT agents}
    % %     \For{$i \in 1, \ldots,n$}
    % %         \State $M_i \gets \textsc{TrainUnsup}(S,T)$ \algorithmiccomment{Train UMT agent}
    % %         \State $\mathcal{M} \gets \mathcal{M}\cup \{M_i\}$
    % %     \EndFor
    % %     % \State $\gD \gets (\varnothing, \varnothing)$ \algorithmiccomment{Initialize pseudo-parallel dataset}
    % %     \State $\mathcal{U} \gets \text{Empty LIFO stack}$ \algorithmiccomment{Initialize agent stack}
    % %     % \State $\gD \gets \gD \cup \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k, M_i^{t\rightarrow s}(T), M_i^{s\rightarrow t}(S))$
    % %     \State $\gD \gets \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k, S, T)$ \algorithmiccomment{Generate synthetic parallel data}
    % %     \State $\hat{M}_{s \rightarrow t} \gets \textsc{TrainSup}(\gD)$  \algorithmiccomment{Train the final model for $s\rightarrow t$}
    % %     \State $\hat{M}_{t \rightarrow s} \gets \textsc{TrainSup}(\gD'=\textsc{Reverse}(\gD))$  \algorithmiccomment{Train the final model for $t\rightarrow s$}
    % %     \State \textbf{return} $\hat{M}_{s \rightarrow t}$, $\hat{M}_{t \rightarrow s}$
    % % \EndProcedure
    % % \end{algorithmic}
    % % % \vspace{-1em}
    % % \end{algorithm}
    
    
    % \begin{algorithm}[t!]
    % % \caption{Positional Encoded Up-sampling: given an image feature map $M$ which has $D$ dimensions resolution $S$ and $C$ channels, return up-sampled image feature map $M'$ that has resolution $2S$}
    % %\small
    % \footnotesize
    % \caption{MACD: Given monolingual data $X_{l_1}$ and $X_{l_2}$ of languages $l_1$ and $l_2$, return a UMT model with parameter $\hat{\theta}$.}
    % \label{alg:macd}
    % \begin{algorithmic}[1]
    % \Procedure{MACD}{$S,T,n,k$}
    %     % \State $\mathcal{M} \gets \varnothing$ \algorithmiccomment{Set of UMT agents}
    %     \State Train 1st unsupervised agent with parameter $\theta_1$
    %     \State Train 2nd unsupervised agent with parameter $\theta_2$
    %     \State Randomly initialize parameter $\hat{\theta}$
    %     \While{until convergence}
    %         \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_1,\theta_2, s, t, \hat{\theta})$
    %         \State $\hat{\theta} \gets \hat{\theta} - \eta \nabla_{\hat{\theta}} \mathcal{L}(\theta_2,\theta_1, s, t, \hat{\theta})$
    %         % \For{$\theta_{\alpha},\theta_{\beta} \in [\{\theta_1,\theta_2\},\{\theta_2,\theta_1\}]$}
    %         %     \State Sample $x_s$, $x_t$ from $X_{s}$ and $X_{t}$
    %         %     \State $y_s \sim P(\cdot|x_s,\theta_{\alpha},s,t)$, $y_t \sim P(\cdot|x_t,\theta_{\alpha},t,s)$
    %         %     \State $\hat{\theta} \gets \hat{\theta} + \eta \nabla_{\hat{\theta}}\log P(y_s|x_s, \hat{\theta},s,t)$
    %         %     \State $\hat{\theta} \gets \hat{\theta} + \eta \nabla_{\hat{\theta}}\log P(x_t|y_t, \hat{\theta},s,t)$
    %         %     \State $z_s \sim P(\cdot|y_s,\theta_{\beta},t,s)$, $z_t \sim P(\cdot|y_t,\theta_{\beta},s,t)$
    %         %     \State $\hat{\theta} \gets \hat{\theta} + \eta \nabla_{\hat{\theta}}\log P(y_s|z_s, \hat{\theta},s,t)$
    %         %     \State $\hat{\theta} \gets \hat{\theta} + \eta \nabla_{\hat{\theta}}\log P(z_t|y_t, \hat{\theta},s,t)$
    %         % \EndFor
    %         % \For{$s, t \in [\{l_1,l_2\}, \{l_2,l_1\}]$}
    %         %     % \For{$s$}
    %         %     \State Sample $x$ from $X_{s}$
    %         %     \State $y^{1} \sim P(\cdot|x,\theta_1,s,t)$, $z^{12} \sim P(\cdot|y^{1},\theta_2,t,s)$
    %         %     \State $y^{2} \sim P(\cdot|x,\theta_2,s,t)$, $z^{21} \sim P(\cdot|y^{1},\theta_1,t,s)$
    %         %     \State $\hat{\theta}_{st} \gets \hat{\theta}_{st} + \eta \nabla_{\hat{\theta}_{st}}\log P(y^1|x, \hat{\theta}_{st},s,t)$
    %         %     \State $\hat{\theta}_{st} \gets \hat{\theta}_{st} + \eta \nabla_{\hat{\theta}_{st}}\log P(y^1|x, \hat{\theta}_{st},s,t)$
    %         %     \State $\hat{\theta}_{st} \gets \hat{\theta}_{st} + \eta \nabla_{\hat{\theta}_{st}}\log P(y^1|z^{12}, \hat{\theta}_{st},s,t)$
    %         %     \State $\hat{\theta}_{st} \gets \hat{\theta}_{st} + \eta \nabla_{\hat{\theta}_{st}}\log P(y^2|z^{21}, \hat{\theta}_{st},s,t)$
    %         %     \State $\hat{\theta}_{ts} \gets \hat{\theta}_{ts} + \eta \nabla_{\hat{\theta}_{ts}}\log P(x|y^1, \hat{\theta}_{ts},t,s)$
    %         %     \State $\hat{\theta}_{ts} \gets \hat{\theta}_{ts} + \eta \nabla_{\hat{\theta}_{ts}}\log P(x|y^1, \hat{\theta}_{ts},t,s)$
    %         %     \State $\hat{\theta}_{ts} \gets \hat{\theta}_{ts} + \eta \nabla_{\hat{\theta}_{ts}}\log P(z^{12}|y^1, \hat{\theta}_{ts},t,s)$
    %         %     \State $\hat{\theta}_{ts} \gets \hat{\theta}_{ts} + \eta \nabla_{\hat{\theta}_{ts}}\log P(z^{21}|y^2, \hat{\theta}_{ts},t,s)$
    %         % \EndFor
    %         % \State Sample batch $X$ from $S$, $Y$ from $T$
    %         % \State $Y^{1} \sim P(Y|X, \theta_1)$, $Y^{2} \sim P(Y|X, \theta_2)$
    %         % \State $X^{1} \sim P(X|Y, \theta_1)$, $X^{2} \sim P(X|Y, \theta_2)$
    %         % \State $X^{12} \sim P(X|Y^{1}, \theta_2)$, $X^{21} \sim P(X|Y^{2}, \theta_1)$
    %         % \State $Y^{12} \sim P(Y|X^{1}, \theta_2)$, $Y^{21} \sim P(Y|X^{2}, \theta_1)$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y^{1}|X, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y^{2}|X, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y|X^{1}, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y|X^{2}, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y^{12}|X^{1}, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y^{21}|X^{2}, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y^{1}|X^{12}, \theta_{st})$
    %         % \State $\theta_{st} \gets \theta_{st} - \eta \nabla_{\theta_{s t}}\log P(Y^{2}|X^{21}, \theta_{st})$
    %     \EndWhile
    %     % \For{$i \in 1, \ldots,n$}
    %     %     \State $M_i \gets \textsc{TrainUnsup}(S,T)$ \algorithmiccomment{Train UMT agent}
    %     %     \State $\mathcal{M} \gets \mathcal{M}\cup \{M_i\}$
    %     % \EndFor
    %     % % \State $\gD \gets (\varnothing, \varnothing)$ \algorithmiccomment{Initialize pseudo-parallel dataset}
    %     % \State $\mathcal{U} \gets \text{Empty LIFO stack}$ \algorithmiccomment{Initialize agent stack}
    %     % % \State $\gD \gets \gD \cup \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k, M_i^{t\rightarrow s}(T), M_i^{s\rightarrow t}(S))$
    %     % \State $\gD \gets \textsc{Recur\_MACD}(\mathcal{M}, \mathcal{U}, n, k, S, T)$ \algorithmiccomment{Generate synthetic parallel data}
    %     % \State $\hat{M}_{s \rightarrow t} \gets \textsc{TrainSup}(\gD)$  \algorithmiccomment{Train the final model for $s\rightarrow t$}
    %     % \State $\hat{M}_{t \rightarrow s} \gets \textsc{TrainSup}(\gD'=\textsc{Reverse}(\gD))$  \algorithmiccomment{Train the final model for $t\rightarrow s$}
    %     \State \textbf{return} $\hat{\theta}$
    % \EndProcedure
    % \end{algorithmic}
    % % \vspace{-1em}
    % \end{algorithm}
    
    
    
    % % \ref{algo:macd_general}
    % % The MACD strategy can be generalized to the $k^{\text{th}}$ level. However, for the sake of brevity and the scope of our experiments, we only describe the second level variant in this paper. We provide a recursive algorithm and other details for the $k^{\text{th}}$ level generalized MACD in the Appendix. 
    % %$s\rightarrow t$ 
    
    % \alert{Rename cross-translation to something else, and rename MACD}
    % In the MACD strategy (\Cref{alg:macd}), at each step, each agent $\theta \in \Theta=\{\theta_1,\theta_2\}$ samples translations from the monolingual data of both languages $l_1$ and $l_2$ to acquire \emph{first level} synthetic parallel data $y$. In the second level, the other agent $\Theta \setminus \theta$ is used to sample the translation $z$ of the translation $y$ of $x$. This process is basically back-translation, but with the backward model coming from a different regime than that of the forward model. The fact that the first level agent must be different from the second level agent is crucial to achieve desirable level of diversity in data generation. After this, we update the final model $\hat{\theta}$ with synthetic pairs $(x,y)$ and $(y,z)$ with maximum likelihood estimation (MLE).
    
    % % The MACD strategy (\Cref{alg:macd}) first sets up an empty \emph{supervised} dataset, $\gD=(\varnothing, \varnothing)$. Then, each agent $M_i$ performs translations from the monolingual data of both sides $S$ and $T$ to acquire synthetic parallel data $(S, M_i^{s\rightarrow t}(S))$ and $(M_i^{t\rightarrow s}(T), T)$, which are then added to $\gD$. Since at this stage only one UMT agent is used to generate the synthetic dataset, this stage is defined as the first level of diversification. In the second level, for each agent $M_i$, another agent $M_j$ ($M_i \neq M_j$) is deployed to translate the \emph{translations} by $M_i$ back to the original language. This process is basically {back-translation}, but with the backward model $M_j$ coming from a different regime than that of the forward model $M_i$. The fact that $M_j$ must be different from $M_i$ is {indeed crucial to achieve diversity in data generation} and the reason why our method is called ``cross-translated''. We then add this second level of synthetic parallel data (which no longer contain the real monolingual data) to the dataset $\gD$. More specifically, in the second level, dataset $\gD$ is appended with $(M_j^{t\rightarrow s}(M_i^{s\rightarrow t}(S)), M_i^{s\rightarrow t}(S))$ and $(M_i^{t\rightarrow s}(T), M_j^{s\rightarrow t}(M_i^{t\rightarrow s}(T)))$. The process goes on where the agents at the $k$-{\text{th}} level translate the products of their counterparts at level $k-1$. In the final step, we train a newly supervised MT model on this augmented data. Algorithm \ref{alg:macd} outlines the entire process of MACD.     
    
    %   %those synthetic parallel data, which now no longer contain the real monolingual data, to the dataset $\gD$. 
      
    %       %$(k-1)^{\text{th}}$ level counterparts. 
          
    % % \ie\
    % % It is worth noting that the total size of the synthetic parallel data grows quadratically with regard to the multiplier $n$ in second level MACD, cubically in the third level, and so on. More accurately, assuming the sizes of monolingual data $S$ and $T$ are equal (\textit{i.e.,} $|S|=|T|$), the total data size $|\gD|$ is:
    % % \begin{equation}
    % %     |\gD| = |S|\left( 2\sum_{i=1}^k \Myperm{k} \right) = 2|S| \sum_{i=1}^k \frac{n!}{(n-k)!} \label{eqn:data_size}
    % % \end{equation}
    % %where $P(n,k)$ is the $k$-permutations of $n$. 
    
    % \red{On one hand, this is favourable for a supervised NMT model which is inherently data hungry and performs well on very large dataset. Nonetheless, one may argue that such model only performs well on a dataset with minimal duplicates, whereas $\gD$ is prone to be overwhelmed with duplicates because there is no additional real data sources and the UMT agents just translate the monolingual data back and forth. In our experiments, on the contrary, the dataset $\gD$ contains only around 14\% duplicates across different language pairs. We show our analysis on data diversity in Section \ref{subsec:data_diversity}.
    % }
    


==> img/Srel-works.tex <==
% There has long been a desire to make use of vast monolingual data to boost MT quality. The first step towards this direction is semi-supervised training. Back-translation \citep{backtranslate_sennrich-etal-2016-improving,understanding_backtranslation_scale} is an effective approach to exploit target-side monolingual data. \citet{iterative-hoang-etal-2018} propose iterative back-translation to further improve it. Dual learning \citep{duallearning_he2016dual,multiagent}, meawhile, is an attractive alternative where the {backward and forward models} are trained concurrently and intertwined with each other. Recently, \citet{mirror_Zheng2020Mirror-Generative} proposed a variational method to couple the translation and language models {through a shared latent space} to train from both parallel and monolingual data {simultaneously}. {There have also been attempts in solving low-resource translation problems with limited parallel data \citep{uni_nmt_low_resource_gu2018universal,hallucinating_phrase_lowrs_mt_irvine2014hallucinating,flores}.} In the realm of SMT, cross-lingual dictionaries have been leveraged to reduce parallel data reliance \citep{end2end_smt_small_data_irvine2016end,hallucinating_phrase_lowrs_mt_irvine2014hallucinating,smt_without_parallel_klementiev2012toward}.

% reduced version
% There has long been a desire to make use of vast monolingual data to boost MT quality. The first step towards this direction is semi-supervised training. 
The first step towards utilizing the vast monolingual data to boost MT quality is through semi-supervised training.
Back-translation \citep{backtranslate_sennrich-etal-2016-improving,understanding_backtranslation_scale} is an effective approach to exploit target-side monolingual data. Dual learning \citep{duallearning_he2016dual,multiagent}, meanwhile, trains {backward and forward models} concurrently and intertwines them together. Recently, \citet{mirror_Zheng2020Mirror-Generative} proposed a variational method to couple the translation and language models {through a shared latent space}.
% to train from both parallel and monolingual data {simultaneously}. 
{There have also been attempts in solving low-resource translation problems with limited parallel data \citep{uni_nmt_low_resource_gu2018universal,hallucinating_phrase_lowrs_mt_irvine2014hallucinating,flores}.} In the realm of SMT, cross-lingual dictionaries have been used to reduce parallel data reliance \citep{end2end_smt_small_data_irvine2016end,smt_without_parallel_klementiev2012toward}.

% \citet{iterative-hoang-etal-2018} propose iterative back-translation to further improve it.

% perhaps we don't need to elaborate much from these papers. Ok, I'm just concerned about space. You're right. But, should I include as many citations because I afraid they will demand us to cite those papers. Or should I focus on a few and elaborate them.

% this is not a good practice to just name the problem; you should at least give some idea what was done (in method), otherwise what's the point of having a related work. If I read a related work and don't get any idea what was done, how can I compare with that.. 

%translation  and language modeling models 
% Fully unsupervised machine translation is even more challenging. \citet{ravi2011deciphering} proposed unsupervised techniques for PBSMT. In recent years, \citet{muse_conneau2017word} proposed MUSE, which is an unsupervised word-translation system that is able to align word embeddings from one language to another by training domain-adversarial objective. 

% \blue{

% }



% \citep{song2019mass}

% In recent years, unsupervised word-translation via cross-lingual word embedding has seen a huge success  \citep{muse_conneau2017word,bilingual_word_embed_artetxe2017learning,Artetxe-2018-acl}.
% This opened the door for UMT methods that employ the three principles described in \cref{sec:background}. \citet{lample2017unsupervised} and \citet{unmt_artetxe2018unsupervised} were among the first of this kind, who use denoising autodecoder for language modeling and iterative back-translation.
% \citet{lample2017unsupervised} use MUSE \citep{muse_conneau2017word} as the initialization to bootstrap the UMT model, while \citet{unmt_artetxe2018unsupervised} use cross-lingual word embeddings \citep{bilingual_word_embed_artetxe2017learning}.
% \citet{lample2018phrase_unsup} later suggested the use of BPE \citep{sennrich2015neural} and fastText \citep{fasttext} to initialize the model and the parameters sharing. Pretrained language models \citep{devlin2018bert} are then used to initialize the entire network \citep{conneau2019cross_xlm}. \citet{song2019mass} proposed to pretrain an encoder-decoder model while \citet{unsup_smt_artetxe-etal-2018-unsupervised} suggested a combination of PBSMT and NMT with subword information.\footnote{Since \citet{unsup_smt_artetxe-etal-2018-unsupervised} did not provide the code, we were unable to apply CBD to their work.} Plus, pretraining {BART \citep{lewis-etal-2020-bart}} on multi-lingual corpora improves the initialization process \citep{mbart_liu2020multilingual}.


% Our proposed CBD works outside the three-principle UMT framework and is considered as an add-on to any underlying UMT system. There exist some relevant approaches to CBD. First, it is similar to \citet{nguyen2019data}, which generates a diverse set of data from multiple \emph{supervised} MT agents. Despite being effective in supervised and semi-supervised settings, a direct implementation of it in UMT underperforms due to lack of supervised signals (\cref{subsec:cross_translation}). In order to successfully exploit unsupervised agents, CBD requires cross-model back-translation which is the key to its effectiveness. Second, CBD can be viewed as an augmentation technique \citep{data_aug_low_resource_fadaee-etal-2017-data,switchout}. Although the denoising autoencoding built in a typical UMT system also performs augmentation, the noising process is rather naive, while CBD augments data by well-trained agents.  
% Third, CBD is related to ensemble knowledge distillation \citep{knowledge_distill_kim_rush_2016,ensemble_distill_freitag2017}. However, these distillation schemes only apply to supervised settings and the agents are used to jointly produce high quality translations rather than diverse candidates. Multi-agent dual learning \citep{multiagent} is also relevant as it seeks to minimize the reconstruction losses using multiple agents. 

In recent years, unsupervised word-translation via cross-lingual word embedding has seen a huge success  \citep{muse_conneau2017word,bilingual_word_embed_artetxe2017learning,Artetxe-2018-acl}.
This opened the door for UMT methods that employ the three principles described in \cref{sec:background}. \citet{lample2017unsupervised} and \citet{unmt_artetxe2018unsupervised} were among the first of this kind, who use denoising autodecoder for language modeling and iterative back-translation.
\citet{lample2017unsupervised} use MUSE \citep{muse_conneau2017word} as the initialization to bootstrap the model, while \citet{unmt_artetxe2018unsupervised} use cross-lingual word embeddings \citep{bilingual_word_embed_artetxe2017learning}.
\citet{lample2018phrase_unsup} later suggested the use of BPE \citep{sennrich2015neural} and fastText \citep{fasttext} to initialize the model and the parameters sharing. Pretrained language models \citep{devlin2018bert} are then used to initialize the entire network \citep{conneau2019cross_xlm}. \citet{song2019mass} proposed to pretrain an encoder-decoder model while \citet{unsup_smt_artetxe-etal-2018-unsupervised} suggested a combination of PBSMT and NMT with subword information.\footnote{Since \citet{unsup_smt_artetxe-etal-2018-unsupervised} did not provide the code, we were unable to apply CBD to their work.} Plus, pretraining {BART \citep{lewis-etal-2020-bart}} on multi-lingual corpora improves the initialization process \citep{mbart_liu2020multilingual}.

% revision
Our proposed CBD works outside the three-principle UMT framework and is considered as an add-on to any underlying UMT system. There exist some relevant approaches to CBD. First, it is similar to \citet{nguyen2019data}, which generates a diverse set of data from multiple \emph{supervised} MT agents. Despite being effective in supervised and semi-supervised settings, a direct implementation of it in UMT underperforms due to lack of supervised signals (\cref{subsec:cross_translation}). In order to successfully exploit unsupervised agents, CBD requires cross-model back-translation which is the key to its effectiveness. Second, CBD can be viewed as an augmentation technique \citep{data_aug_low_resource_fadaee-etal-2017-data,switchout}. Although the denoising autoencoding built in a typical UMT system also performs augmentation, the noising process is rather naive, while CBD augments data by well-trained agents.  
Third, CBD is related to ensemble knowledge distillation \citep{knowledge_distill_kim_rush_2016,ensemble_distill_freitag2017}. These methods use multiple models to perform ensemble inference to generate one-way synthetic targets from the original source data, which are then used to distill the final model. However, these distillation schemes only apply to supervised settings and the agents are used to jointly produce high quality translations rather than diverse candidates. Similar to our method, multi-agent dual learning \citep{multiagent} also uses multiple models in both forward and backward directions, but to minimize the reconstruction losses instead of to generate diverse synthetic data.







==> img/macro.tex <==
\newcommand{\comm}[1]{\textcolor{blue}{\noindent #1}}
\newcommand{\alert}[1]{\textcolor{red}{\noindent$\Rightarrow$ #1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\add}[1]{\textcolor{black}{#1}}


%% abbr 
\newcommand{\ie}{{\em i.e.,}\xspace}
\newcommand{\eg}{{\em e.g.,}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\aka}{\emph{a.k.a.}\xspace}
\newcommand{\resp}{\emph{resp.}\xspace}


\newcommand{\pos}{${pos}$}


%%% inline lists
\newcommand{\Ni}{({\em i})~}
\newcommand{\Nii}{({\em ii})~}
\newcommand{\Niii}{({\em iii})~}
\newcommand{\Niv}{({\em iv})~}
\newcommand{\Nv}{({\em v})~}
\newcommand{\Na}{({\em a})~}
\newcommand{\Nb}{({\em b})~}
\newcommand{\Nc}{({\em c})~}
\newcommand{\Nd}{({\em d})~}
\newcommand{\Ne}{({\em e})~}
\newcommand{\Nf}{({\em f})~}



==> img/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}
\newcommand{\Myperm}[2][^n]{\prescript{#1\mkern-3mu}{}P_{#2}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\makeatletter
\newcommand{\xRightarrow}[2][]{\ext@arrow 0359\Rightarrowfill@{#1}{#2}}
\makeatother


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}
\def\real{{\mathbb{R}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

